LLM-Enhanced Data Management

Machine learning (ML) techniques for optimizing data management problems have been extensively studied and widely deployed in recent five years. However traditional ML methods have limitations on generalizability (adapting to different scenarios) and inference ability (understanding the context). Fortunately, large language models (LLMs) have shown high generalizability and human-competitive abilities in understanding context, which are promising for data management tasks (e.g., database diagnosis, database tuning). However, existing LLMs have several limitations: hallucination, high cost, and low accuracy for complicated tasks. To address these challenges, we design LLMDB, an LLM-enhanced data management paradigm which has generalizability and high inference ability while avoiding hallucination, reducing LLM cost, and achieving high accuracy. LLMDB embeds domain-specific knowledge to avoid hallucination by LLM fine-tuning and prompt engineering. LLMDB reduces the high cost of LLMs by vector databases which provide semantic search and caching abilities. LLMDB improves the task accuracy by LLM agent which provides multiple-round inference and pipeline executions. We showcase three real-world scenarios that LLMDB can well support, including query rewrite, database diagnosis and data analytics. We also summarize the open research challenges of LLMDB.

==> 02-overview.tex <==
%!TEX root = ../main.tex


\vspace{-1em}

\section{The Vison of \oursys}
\label{sec:overview}

%We aim to build a \llm-centric database adminstrator, empowered by \llms and the rich documents. However, 

Existing \llms are criticized for problems like ``Brain in a Vat''~\cite{DBLP:journals/corr/abs-2307-03762}. Thus, it is essential to establish close connections between \llms and the target database, allowing us to guide \llms in effectively maintaining the database's health and functionality. Hence, we propose \oursys, which is composed of two stages. 

%  (e.g., using monitoring metrics and tools)

First, in preparation stage, \oursys generates experience (from documents) and prompt template (from diagnosis samples), which are vital to guide online maintenance. 

%. For the database maintenance problem, they cannot easily build connections of ``words'' and the ``real world database problems'' by itself. That is, they are developed from the batch training data, whose reasoning way may be completely different from that of a human beginner in database maintenance. Human beginners learn from the ``diagnosis steps'' and ``real examples'', while \llms are mainly based the ``token similarity'' captured by the attention mechanism. Besides, caused by the batch training mode, \llms cannot easily synchronize the up-to-date  maintenance knowledge (e.g., system view updates) by updating the model parameters.


\begin{compactitem}
	\item
	\bfit{Documents $\rightarrow$ Experience.} Given a large volume of diverse, long, unstructured  database documents (e.g., database manual,  white paper, blogs), we first split each document into chunks that can be processed by the \llm. To aggregate correlated chunks together (e.g., chunk $v_i$ that explains the meaning of ``bloat-table'' and chunk $v_j$ that utilizes ``bloat-table'' in root cause analysis), we generate a summary for each chunk based on both its content and its subsections. Finally, we utilize \llm to extract maintenance experience from chunks with similar summaries (Section~\ref{sec:prepare}).
	
	\item
	\bfit{Prompt Template Generation.} To help \llm better understand the \dm tasks, we iteratively generate and score different formats of task descriptions using \dm samples (i.e., given the anomaly and solutions, ask \llm to describe the task), and adopt task description that both scores high performance and is sensible to human DBAs (in cases of learning bias) for \llm diagnosis (Section~\ref{sec:prompt}).
\end{compactitem}

Second, in maintenance stage, given an anomaly, \oursys iteratively reasons the possible root causes by taking advantages of external tools and multi-\llm communications.

\begin{compactitem}
	\item
	\bfit{External Tool Learning.} For a given anomaly, \oursys first matches relevant tools using algorithms like Dense Retrieval. Next, \oursys provides the tool APIs together with their descriptions to the \llm (e.g., function calls in GPT-4). After that, \llm can utilize these APIs to obtain metric values or optimization solutions. For example, in PostgresSQL, \llm can acquire the templates of slowest queries in the {\it pg\_activity} view. If these queries consume much CPU resource (e.g., over 80\%), they could be root causes and optimized with rewriting tool (Section~\ref{sec:tool}).
	
	%To obtain the abnormal metrics (from observation tools) and corresponding solutions (from optimization tools), we first utilize algorithms like BM25 and Dense Retrieval to select desired tools (e.g., views for outlining slow queries). Next, we provide \llm with descriptions of the APIs in selected tools ({\it tool query}), and count on \llm to choose required APIs to obtain required metrics or optimization solutions ({\it tool answer}). For example, in Postgres, \llm can acquire the templates of top-5 slow queries in the {\it pg\_activity} view. If these queries consume much CPU resource (e.g., over 80\%), \llm determines they are root causes and calls the rewriting tool to judiciously apply rules to optimize these queries.
	
	\item
	\bfit{\llm Diagnosis.} Although \llm can understand the functions of tool APIs, it still may generate incorrect API requests, leading to diagnosis failures. To solve this problem, we employ the {\it tree of thought} strategy, where \llm can go back to previous steps if the current step fails. It significantly increases the likelihood of \llms arriving at reasonable diagnosis results (Section~\ref{sec:diagnose}).
	
	\item
	\bfit{Collaborative Diagnosis.} A single \llm may execute only the initial diagnosis steps and end up early,  leaving the problem inadequately resolved. To address this limitation, we propose the use of multiple \llms working collaboratively. Each \llm plays a specific role and communicates by the environment settings (e.g., priorities, speaking orders). In this way, we can enable \llms to engage in debates and inspire more robust solutions (Section~\ref{sec:collaborate}). %By leveraging the power of collective intelligence, we can enhance the accuracy and effectiveness of database issue resolutions."
	
\end{compactitem}





\iffalse
\begin{compactitem}
	\item
	\bfit{Knowledge Preparation} \textit{-- Collect the required maintenance metrics, data, and experience}: At this stage, the \llm system prepares itself by gathering all the necessary information to make informed decisions. This includes tracking key maintenance metrics, understanding historical data patterns, and absorbing domain knowledge.
	
	\item
	\bfit{Collaborative Diagnosis \& Optimization} {\it -- Learn diagnosis and optimization knowledge with \llm}: Once anomalies are detected, the \llm leverages learned knowledge and sophisticated algorithms to diagnose potential issues and suggest optimization strategies. This stage embodies the self-healing potential of the system.
	
	\item
	\bfit{Adversarial Experience Accumulation.} {\it -- Solve hybrid root cause problems with the collaboration of  multiple \llms}: In scenarios of complex or multifaceted issues, multiple \llm systems can collaborate, pooling their collective intelligence to identify and solve problems. This collaborative problem-solving strategy offers a robust solution to the ever-increasing complexity of database systems.
\end{compactitem}
\fi

==> 02-preliminary.tex <==
%!TEX root = ../main.tex
\section{Preliminaries}
\label{sec:preliminaries}

\subsection{Large Language Models}

Large language models (LLMs) are a type of machine learning model specifically designed for natural language processing. Most of the current LLMs are based on Transformer~\cite{transformer} architecture, trained on gigantic unlabelled corpora through self-supervised learning tasks, thus possessing the power of understanding natural language. Since GPT-3~\cite{gpt3}, the LLMs are becoming remarkably stronger and have made significant strides in recent years. For instance, the recent ChatGPT~\cite{chatgpt} and GPT-4~\cite{gpt4} have exhibited possession of common sense knowledge, and outstanding ability to reason and perform logical inference tasks with high accuracy. This progress has led to an exponential increase in the number of applications of LLMs in various fields such as natural language generation, question-answering systems, and language translation, among others.

Meanwhile, as the language models become larger in size, their computational cost of large language increased dramatically. As a result, fine-tuning these large models for every downstream task has become impractical. This has sparked interest in a new approach to utilizing LLMs. Prompt-tuning is a general method that enables users to apply LLMs to new tasks and data domains without modifying the models themselves. This is achieved by incorporating prompts, such as descriptions, tags, and learnable components, as textual input to the LLM. Prompt-tuning is a powerful and efficient way of utilizing LLMs. In addition to prompt-tuning, the development of open-source LLMs like LLaMA~\cite{llama} has contributed to the flourishing of delta-tuning, an alternative method for utilizing LLMs. Delta-tuning involves adding extra parameters to the original LLM and updating only these additional parameters while keeping the LLM frozen. Since the number of tuned parameters is typically much smaller than the size of the original LLM, this approach reduces the computational cost and increases efficiency.

\subsection{\todo{???}}

==> 03-knowledge.tex <==
%!TEX root = ../main.tex


\section{Experience Detection From Documents}
\label{sec:prepare}

Document learning aims to extract experience segments from textual sources, where the extracted segments are potentially useful in different \dm cases. For instance, when analyzing the root causes of performance degradation, \llm utilizes the {\it ``many\_dead\_tuples''} experience to decide whether dead tuples have negatively affected the efficiency of index lookup and scans.


\hi{Desired Experience Format.} To ensure \llm can efficiently utilize the experience, each experience fragment should include four fields. As shown in the following example, {\it ``name''} helps \llm to understand the overall function; {\it ``content''} explains how the root cause can affect the database performance (e.g.,  the performance hazards of many dead tuples); {\it ``metrics''} provide hints of matching with this experience segment, i.e., \llm will utilize this experience if the abnormal metrics exist in the ``metrics'' field; {\it ``steps''} provide the detailed procedure of checking whether the root cause exists by interacting with database (e.g., obtaining the ratio of dead tuples and live tuples from table statistics views).
\begin{lstlisting}
"name": "many_dead_tuples",
"content": "If the accessed table has too many dead tuples, it can cause bloat-table and degrade performance",
"metrics": ["live_tuples", "dead_tuples", "table_size", "dead_rate"],
"steps": "For each accessed table, if the total number of live tuples and dead tuples is within an acceptable limit (1000), and table size is not too big (50MB), it is not a root cause. Otherwise, if the dead rate also exceeds the threshold (0.02), it is considered a root cause. And we suggest to clean up dead tuples in time."
\end{lstlisting}

% identify section separators (e.g., headlines or index numbers)
% Next,  we construct a tree ${\tt T}$ to denote the document, where each leaf node contains a chunk, and each internal node ${\tt v}$ represents a section, with its child nodes ${\tt v.children}$ corresponding to subsections. %Internal nodes may or may not contain document contents ${\tt v.content}$, depending on whether a preface outside all subsections exists.
%\textit{Step2: Cascading Summary.} Next, for a chunk $v$ as a node in the tree, we 
% each internal node combines (1) the content of the node and (2) the title and summary of its child nodes, which reflect the document structure and is used as index in the next step.

\hi{\llm for Experience Detection.} It aims to detect experience segments that follow above format. Since different paragraphs within a long document may be correlated with each other (e.g., the concept of ``bloat-table'' appearing in ``many\_dead\_tuples'' is introduced in another section), we explain how to extract experience segments without losing the technical details.

\textit{Step1: Segmentation.} Instead of partitioning documents into fixed-length segments, we divide them based on the structure of the section structures and their content. Initially, the document is divided into chunks using the section separators. If a chunk exceeds the maximum chunk size (e.g., 1k tokens), we further divide it recursively into smaller chunks.

\textit{Step2: Chunk Summary.} Next, for each chunk denoted as $x$, a summary $x.summary$ is created by feeding the content of $x$ into \llm with a summarization prompt $p_{summarize}$:

\begin{tcolorbox}[enhanced,sharp corners,
	width={8.5cm},
	colback=white,
	borderline={0.3mm}{0.3mm}{white},
	boxsep=-.5mm]
	\bfit{$p_{summarize}$} = {\it Summarize the provided chunk briefly $\cdots$ Your summary will serve as an index for others to find technical details related to database maintenance $\cdots$ Pay attention to examples even if the chunks covers other topics.}
\end{tcolorbox}

The generated $x.summary$ acts as a textual index of $x$, enabling the matching of chunks containing similar content.

\textit{Step3: Experience Extraction.} Once the summaries of the chunks are generated, \llm parses the content of each chunk and compares it with the summaries of other chunks having similar content, which is guided by the extraction prompt $p_{extract}$. This way, experience segments that correlate with the key points from the summaries are detected.


\begin{figure*}[!t]
	\centering
	\includegraphics[width=.98\linewidth]{./figures/knowledge2.png}
	\vspace{.5em}
	\captionsetup{skip=0pt}
	\caption{The outline of diagnosis experience extracted from documents.}
	\label{fig:knowledge}
	%\vspace{-.5em}
\end{figure*}


\begin{tcolorbox}[enhanced,sharp corners,
	width={8.5cm},
	colback=white,
	borderline={0.3mm}{0.3mm}{white},
	boxsep=-.5mm]
	\bfit{$p_{extract}$} = {\it Given a chunk summary, extract diagnosis experience from the chunk.} {\it If uncertain, explore diagnosis experience in chunks with similar summaries.}
\end{tcolorbox}


In our implementation, given a document, we use \llm to extract experience segments into the above 4-field format.

%In our implementation, we utilize \llm to extract experience segments from a given document and format them into a standardized 4-field structure.

%interacts with ${\tt T}$ to progressively extract diagnosis experience from the documents. The cascading summary automatically responds to inquiries $\{p_{extract}\}$ from the \llm to provide local information for experience extraction. 

 %To facilitate this process, we provide a description of the ``many\_dead\_tuples'' experience, which enables the \llm to directly generate experience that adhere to the similar format.

\hi{Detected Maintenance Experience.} In Figure~\ref{fig:knowledge}, we showcase the simplified diagnosis procedure together with some necessary details, coming from chunks originally in different sections of the given documents (e.g., the maintenance guide with over 100 pages).


{\tt 1. Background Understanding.} It's crucial to grasp the context of system performance, such as recent changes in customer expectation, workload type, or even system settings.

\begin{sloppypar}
{\tt 2. Database Pressure Checking.} This step identifies database bottlenecks, such as  tracking CPU usage and active sessions; and monitoring system views (e.g., \textit{pg\_stat\_activity} and \textit{pgxc\_stat\_activity}) to focus on non-idle sessions. 
\end{sloppypar}

{\tt 3. Application Pressure Checking.} If there is no apparent pressure on the database or the resource consumption is very low (e.g., CPU usage below 10\% and only a few active sessions), it is suggested to investigate the application side, such as exhausted application server resources, high network latency, or slow processing of queries by application servers.


{\tt 4. System Pressure Checking.} The focus shifts to examining the system resources where the database is located, including CPU usage, IO status, and memory consumption. %For CPU-related issues, one can analyze the WDR report's ``Top SQL ordered by CPU Time'' section or generate flame graphs for anomalies in CPU usage. In case of IO-related problems, metrics like `\%util`, `r\_await`, and `w\_await` from `iostat` can be observed. High IO consumption can be attributed to certain SQL queries, which can be identified using `pidstat` and `pg\_thread\_wait\_status` views.

{\tt 5. Database Usage Checking.} Lastly, we can investigate sub-optimal database usage behaviors, such as (1) addressing concurrency issues caused by locking waits, (2) examining database configurations, (3) identifying abnormal wait events (e.g., io\_event), (4) tackling long/short-term performance declines, and (5) optimizing poorly performing queries that may be causing bottlenecks.

%In conclusion, these five steps offer a comprehensive approach to diagnose and address performance issues in the database system effectively. By following this process and utilizing appropriate monitoring tools and views, \llms can pinpoint the root causes and implement targeted optimizations to improve overall system performance.


\iffalse
\begin{itemize}
	
	\item \textbf{SQL Statement Writing Issue}
	\begin{itemize}
		\item Redundant Operators
		\item Complex Calculations
		\item Index Inefficiency (at SQL writing level)
	\end{itemize}
	
	\item \textbf{Optimizer Problems}
	\begin{itemize}
		\item Cardinality Estimation Error
		\item Cost Estimation Error
	\end{itemize}

	\item \textbf{Indexing Reasons}
	\begin{itemize}
		\item Lack of Effective Indexing
		\item Existing Index Becoming Inefficient
		\item Redundant Indexing
	\end{itemize}

	\item \textbf{System Configuration Reasons}
	\begin{itemize}
		\item Memory Space Configuration Issues
		\item Optimizer Configuration Issues
		\item Concurrency Conflict Issues
		\item Execution Efficiency Issues
		\item Background Process Resource Occupation
	\end{itemize}
		
\end{itemize}
\fi



==> 03-related_work.tex <==
%!TEX root = ../main.tex
\section{Related Work}
\label{sec:related_work}

\todo{Related Work}

==> 03-rule.tex <==
%!TEX root = ../main.tex

\section{Preliminaries}
\label{sec:preliminary}

% which anomalies
\hi{Database Anomalies.} In databases, there are five common problems that can negatively affect the normal execution status. {\it (1) Running Slow.} The database exhibits longer response time than expectancy, leading to bad execution performance. {\it (2) Full Disk Capacity.} The database's disk space is exhausted, preventing it from storing new data. {\it (3) Execution Errors.} The database experiences errors, potentially due to improper error handling in the application (e.g., leaking sensitive data or system details) or issues within database (e.g., improper data types). {\it (4) Hanging.} The database becomes unresponsive, which is usually caused by long-running queries, deadlocks, or resource contention. {\it (5) Crashing.} The database unexpectedly shuts down, causing data inaccessible. {\it For a mature database product, each anomaly type is explained in the documentation and suitable to be learned by \llms.}

% according what metrics we analyze the potenial causes of these anomalies


%\hi{Observation tools for anomaly detection.} ``Observability of the database'' is vital to detect above anomalies, including logs, metrics, and traces. \textit{(1) Logs} are records of database events. For example, Postgres supports slow query logs (with error messages that can help debug and solve execution issues), but these logs may record a large scale of data and are generally not enabled in online stage. %They provide detailed context on what happened at a specific point in time and are indispensable in diagnosing errors or unexpected behaviors in the system.  \textit{(2) Metrics} capture the aggregated database and system statistics. For example, views like pg\_stat\_statements record the templates and statistics of slow queries; tools like Prometheus~\cite{turnbull2018monitoring} provide numerous monitoring metrics, making it possible to capture the real time system status. \textit{(3) Traces}  provide visibility into how requests behave during executing in the database. Different from logs that help to identify the database problem, traces help to locate the specific abnormal workload or application. %Since logs and traces are generally costly to use, {\it metrics are most commonly used in detecting the anomalies in initial diagnosis stage.}

%For example, users can use tools like pg\_activity in PostgreSQL to monitor slow queries, which effectively presents a live view of the database server and assists in spotting queries that take an unusually long time to execute. %These traces are invaluable when trying to understand the sequence of operations and the time each operation takes. % They capture the lifetime of a request as it flows through various components of a system, providing a detailed picture of its journey and helping to identify the source of latency issues. One

%\hi{Optimization tools for anomaly solving.} Actually, users only concern how to restore to the normal status after an anomaly occurs. Here we showcase some optimization tools. (1) For slow queries, since most open databases are weak in logical transformation, there are external engines (e.g., around 120 rules in Calcite) and tuning guides (e.g., over 34 transformation suggestions in Oracle) that help to optimize slow queries. (2) For knob tuning, many database failures (e.g., max\_connections in Postgres) or bad performance (e.g., memory management knobs) are correlated with database knobs (e.g., for a slow workload, incresae innodb\_buffer\_pool\_size in MySQL by 5\% if the memory usage is lower than 60\%). Similarly, there are index tuning rules that generate potentially useful indexes (e.g., taking columns within the same predicate as a composite index). Furthermore, we can utilize more advanced methods, such as selecting among heuristic methods~\cite{AutoAdmin,Drop,DB2Advis} and learned methods~\cite{SWIRL,DBABandits,CIKM20,SmartIX,AutoIndex,BudgetMCTS} for problems like {\it index lacking}, which is not within the scope of this paper.

%They provide detailed context on what happened at a specific point in time and are indispensable in diagnosing errors or unexpected behaviors in the system. 


\hi{Observation Tools for Anomaly Detection.} ``Observability of the database'' is vital to detect above anomalies, including logs, metrics, and traces. \textit{(1) Logs} are records of database events. For example, PostgresSQL supports slow query logs (with error messages that can help debug and solve execution issues), but these logs may record a large scale of data and are generally not enabled in online stage. \textit{(2) Metrics} capture the aggregated database and system statistics. For example, views like pg\_stat\_statements record the templates and statistics of slow queries; tools like Prometheus~\cite{turnbull2018monitoring} provide numerous monitoring metrics, making it possible to capture the real time system status. \textit{(3) Traces}  provide visibility into how requests behave during executing in the database. Different from logs that help to identify the database problem, traces help to locate the specific abnormal workload or application. 

%Since logs and traces are generally costly to use, {\it metrics are most commonly used in detecting the anomalies in initial diagnosis stage.}
%For example, users can use tools like pg\_activity in PostgreSQL to monitor slow queries, which effectively presents a live view of the database server and assists in spotting queries that take an unusually long time to execute. %These traces are invaluable when trying to understand the sequence of operations and the time each operation takes. % They capture the lifetime of a request as it flows through various components of a system, providing a detailed picture of its journey and helping to identify the source of latency issues. One

\hi{Optimization Tools for Anomaly Solving.} Users mainly concern how to restore to the normal status after an anomaly occurs. Here we showcase some optimization tools. (1) For slow queries, since most open-source databases are weak in logical transformation, there are external engines (e.g., Calcite with $\sim$120 query rewrite rules) and tuning guides (e.g., Oracle with over 34 transformation suggestions) that help to optimize slow queries. (2) For knob tuning, many failures (e.g., max\_connections in Postgres) or bad performance (e.g., memory management knobs) are correlated with database knobs (e.g., for a slow workload, incresae innodb\_buffer\_pool\_size in MySQL by 5\% if the memory usage is lower than 60\%). Similarly, there are index tuning rules that generate potentially useful indexes (e.g., taking columns within the same predicate as a composite index). Besides, we can utilize more advanced methods, such as selecting among heuristic methods~\cite{AutoAdmin,Drop,DB2Advis} and learned methods~\cite{zhou2020database,SWIRL,DBABandits,CIKM20,SmartIX,AutoIndex,BudgetMCTS} for problems like {\it index lacking}, which is not within the scope of this paper.



We aim to design \oursys, an LLM-based DBA, for automatically diagnosing the database anomalies and use LLM to directly  (or call appropriate tools to indirectly) provide the root causes.





\iffalse
Anomalies is closely relevant to the application scenarios, such as (1) the user reports a high latency wait for the database responses; (2) the performance metrics like 80th/95th percentile are swiftly increasing; (3) many slow queries (e.g., over 1 seconds) occur in last time windows.


Note it is critical to communicate with the users and gain the background information instead of rushing to start diagnosis \& optimization. For example, whether there are changes in performance expectation, workload types, or hardware settings, which can also lead to significant metric value changes but are generally not taken as anomalies.


The performance is slower than a threshold.

Method\#1: The metric is abnormal if exceeding some empirical thresholds  

Method\#2: Compare the similarity of curves within two time periods  (KS-Test)
 Time-series curves $\rightarrow$ CDFs. Compute the maximum absolute difference of the CDFs


Method\#3: Compare the similarity of curves within two time periods  (Encoder-Decoder)

 Based on the an extensive of relevant document collection, we find that $(i)$ the typical anomalies are similar across different database systems but $(ii)$ the way to identify anomalies are quite different. 

First, conceptually

In the context of databases, several anomalies are commonly encountered, encompassed within the realm of slow queries, database configurations, data volume, and indices. Slow queries are often attributed to complicated SQL commands, akin to those found in TPC-H benchmarks, SQL operations that join multiple tables, typical of job databases, or SQL queries handling high concurrency, which can be simulated by tools such as sysbench. Anomalies within database configurations are frequently due to a limited degree of concurrency, indicated by an exceedingly low `max\_connections` parameter, or insufficient memory allocation, as defined by parameters like `shared\_buffer` or `work\_mem`. Moreover, data volume anomalies are frequently caused by configurations that define an excessively large size. Finally, inconsistencies related to indices, whether missing or surplus, lead to inefficient database operations. These areas collectively constitute the most typical sources of anomalies within a database environment.

\fi

%\hi{Anomalies.} The generation of anomalous scenarios in databases often involves slow queries, database configuration, data volume, and indices. Slow queries can be the result of complicated SQL commands such as those found in TPC-H benchmarks, multiple table join SQL operations often seen in job-related databases, or high concurrency SQL, as tested by tools like sysbench. Database configuration anomalies can occur due to an insufficient level of concurrency, such as when the 'max\_connections' parameter is set too low, or inadequate memory allocation specified by parameters like 'shared\_buffer' or 'work\_mem'. Excessive data volume is another common anomaly, where the configured size is exceedingly large, resulting in performance issues. Lastly, issues related to indices - either missing or redundant - can lead to inefficient database operations. These are some of the typical issues that contribute to abnormal scenarios in a database environment.

==> 04-design.tex <==
%!TEX root = ../main.tex
\section{\sys System Design}
\label{sec:system-design}

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.6\linewidth]{figs/abstraction.pdf}
  \caption{Abstraction illustration.}
  \Description{\sys consists of five layers of abstraction.}
  \label{fig:abstraction}
\end{figure}

The \sys system is designed with a five-layer abstraction to facilitate efficient and effective data science applications. The layers in a top-to-bottom hierarchy include user application, high-level logical operator, low-level logical operator, physical operator, and implementation.

Taking the task of extracting people's names from website titles as a specific example. The high-level logical operator is a data science functionality with certain generality. In this case, an \texttt{EXTRACT} operator, which is configured with specific parameters, such as task description, input/output specifications, and the object to extract (i.e., "names"), all of which could be set by the users in simple natural language.

However, applying one high-level logical operator to all scenarios through the same low-level implementation would not be efficient or effective. To address this, \sys provides multiple alternative choices of low-level logical operators, each offering a different logical implementation pipeline consisting of a series of physical operators. These physical operators are decoupled from their actual implementations, allowing \sys to automatically optimize each physical operator and compile each of them into different implementations depending on specific task instances. The compilation and debugging of the physical operators are completed mostly within the \sys system and boosted by the power of LLMs.

% \todo{Workflow illustration. Replace this one. System architecture + data flow (highlight components, inputs, outputs, separately).}

\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/illustration.pdf}
  \caption{Illustration.}
  \Description{Users only need to communicate with \sys, while \sys coordinates LLMs, data, and tools to generate an efficient and effective local solution.}
  \label{fig:illustration}
\end{figure}

In the \sys study, various methods of employing LLMs in data science applications were investigated, focusing on two primary uses: direct query and code generation. Direct query treats each operator as a black-box function $f:X \to Y$, predicting the output $Y$ from input $X$ in zero-shot or few-shot settings. Code generation necessitates LLMs to create an executable program $r_f$ (e.g., in Python) that corresponds to $f$ for every input-output pair $(X,Y)$, expecting $r_f \equiv f$. The direct query typically assesses the effectiveness of incorporating LLMs, while code generation is employed for greater efficiency, as the executable $r_f$ runs locally. To further enhance LLM utilization, \sys employs a strategy that prioritizes localized computation through a series of optimizer modules: cacher, validator, simulator, ensembler, and adaptor. These modules allow \sys to develop an LLM-powered local solution for improved results. Additionally, \sys incorporates inter-operator optimizations such as predicate pushdown and path compression. Beyond primary uses, \sys explores other LLM applications, including suggestion, planning, and miscellaneous techniques to increase their utility. Furthermore, \sys tackles automatic local data processing with LLMs, encompassing data preprocessing for both LLMs and humans, data generation, and data annotation.

In subsequent chapters, we will examine each LLM utilization approach in detail and discuss specific techniques for optimizing LLM usage in relevant cases.

==> 04-prompt.tex <==
%!TEX root = ../main.tex

\section{Diagnosis Prompt Generation}
\label{sec:prompt}

Instead of directly mapping extracted experience to new cases, next we explore how to teach \llms to (1) understand the database maintenance tasks and (2) reason over the root causes by itself.

% with suitable instructions and demonstration examples. After that, \llms can
% As the saying goes ``{\it giving fish to someone is not better than teaching someone to fish}''. Next 
%utilize external tools and judiciously look up prepared experience 

%\hi{Diagnosis with reasoning.} 
\hi{Input Enrichment.} With a database anomaly $x$ as input, we can enrich $x$ with additional description information so called input prompt $x'$. On one hand, $x'$ helps \llm to better understand the task intent. On the other hand, since database diagnosis is generally a complex task that involves multiple steps, $x'$ preliminarily implies how to divide the complex task into sub-tasks in a proper order, such that further enhancing the reasoning of \llm.

%  and the reasoning trace for finding the root causes or optimization solutions

From our observation, the quality of $x'$ can greatly impact the performance of \llm on maintenance tasks~\cite{Zhou2022a} (Figure~\ref{fig:overview}). Thus, we first utilize \llm to suggest candidate prompts based on a small set of input-output pairs (e.g., 5 pairs for a prompt). Second, we rank these generated prompts based on a customized scoring function (e.g., the ratio of detected root causes), and reserve the best prompts (e.g., top-10) as candidates. Finally, we select the best one to serve as the input prompt template for the incoming maintenance tasks.

% we first automatically generate proper $x'$ with a limited number of diagnosis  samples~\cite{Zhou2022a,Honovich2022}. That is, 

\iffalse
\begin{tcolorbox}[enhanced,sharp corners,
	width={8.3cm},
	colback=white,
	borderline={0.3mm}{0.3mm}{white},
	boxsep=-.5mm]
	\bfit{$p_{diagnosis}$} = {\it You are in a company whose databases meet anomalies and it depends on you to diagnose the root causes.} 
	{\it First, obtain time period the anomaly and memorize the start and end time of the anomaly.} 
	{\it Second, diagnose the causes of the anomaly.} 
	{\it Third, you need to match each cause with potential solutions cached in the knowledge base.} 
	{\it Finally, list the above diagnosed causes and their matched solutions in easy-to-understand format using bullet points.}\\
	--------------------------------\\
	{\it [Demonstration examples]}
	%{\it You are in a company whose databases meet anomalies and it depends on you to diagnose the root causes and their solutions $\cdots$     *Rules and Format Instructions for Response* $\cdots$}
\end{tcolorbox}
\fi

==> 04-tool.tex <==
%!TEX root = ../main.tex

\section{External Tool Learning}
\label{sec:tool}


% In addition to understanding maintenance tasks and processing procedures, an essential aspect of improving database diagnosi
%\textbf{Enhancing Database Diagnosis with External Tools.} We aim to teach \llm to leverage external tools effectively, thereby 

%External tools can broaden the functionality of \llm in database maintenance. 
As we know, the efficient use of tools is a hallmark of human cognitive capabilities~\cite{qin2023tool,qin2023toolllm}. When human beings encounter a new tool, they start to understand the tool and explore how it works, i.e., taking it as something with particular functions and trying to understand what the functions are used for. Likewise, we aim to inspire similar ability within \llm.

\hi{Tool Retrieval.} We first retrieve the appropriate tools for the diagnosis task at hand, represented as $D_t$. There are several methods used, such as BM25, \llm Embeddings, and Dense Retrieval.  

{\it (1) BM25}, simply represented as $f(D_t, Q) = \text{BM25}$, is a common probabilistic retrieval method that ranks tool descriptions ($D$) based on their relevance to the given anomaly ($Q$)~\cite{robertson2009probabilistic}. 

{\it (2) \llm Embeddings}, denoted as $f(D_t, L) = {LLM}_E$, are a method that converts tool descriptions ($D_t$) into embeddings ($E_t$) using \llm, i.e., $E_t = L(D_t)$. These embeddings capture the semantic meanings in a multi-dimensional space, hence helping in finding related tools even in the absence of keyword overlap, $D_t = LLM_E(E_t)$. 

{\it (3) Dense Retrieval}, denoted as $f(Q, D_t, N) = D_R$, uses neural networks ($N$) to generate dense representations of both the anomaly ($Q$) and the tool descriptions ($D_t$), separately denoted as  $\text{Dense}_Q$ and $\text{Dense}_D$. To retrieve the relevant tools, we calculate the similarity between $\text{Dense}_Q$ and $\text{Dense}_D$, and rank them based on these similarity scores.


The proper method for tool retrieval depends on the specific scenarios. {\it BM25} is efficient for quick results with large volumes of API descriptions in the tools and clear anomaly characters. {\it \llm Embeddings} excel at capturing semantic and syntactic relationships, which is especially useful when relevance isn't obvious from keywords (e.g., different metrics with similar functions). {\it Dense Retrieval} is ideal for vague anomaly, which captures context and semantic meaning, but is more computational costly.

%\textit{API Calling.} Query construction plays a vital role in generating data for the tool learning process. Two primary types of queries can be formulated: single API queries and multi-API queries. (1) Single API Query Generation: This involves creating queries for individual APIs. Three main approaches are used for generating these queries: zero-shot query, ICL query, and ICL + observation. Zero-shot query generation entails crafting queries without prior knowledge of the API or its capabilities. ICL query generation employs an Inverse Cloze Task (ICL) approach to generate queries based on the API's documentation. Combining the ICL approach with observations of the API's behavior results in ICL + observation query generation.  (2) Multi-API Query Generation: This process involves generating queries involving multiple APIs. These queries can include APIs from the same tool, different tools within the same category, or even different tools from distinct categories. The specific approach for generating these queries is tailored to the specific requirements of the database diagnosis task.

%\textit{Answer Construction.} During the final stage of database diagnosis, crucial insights are gleaned from the data obtained through queries. To provide actionable solutions, various approaches come into play. For instance, when diagnosing a performance issue in a database, observations can be condensed to highlight the key performance metrics and bottlenecks affecting its efficiency. Retaining historical data, even with corrected errors, enables \llm to identify recurring patterns and optimize database performance in the long run. When dealing with potential API failures, simulating API results aids in predicting potential outcomes, empowering \llm to propose strategies for mitigating errors proactively. Furthermore, incorporating Monte-Carlo Search allows \llm to explore different execution paths, which is particularly useful when diagnosing complex database issues with multiple possible causes. Suppose the database is encountering data inconsistencies. By converting the chain-of-thought into a tree-of-thought approach, \llm can better visualize the relationships between different data entities, leading to more comprehensive diagnoses and recommendations.


==> 05-feedback.tex <==
%!TEX root = ../main.tex

\begin{figure}[!t]
	\vspace{.5em}
	\centering
	\includegraphics[width=.98\linewidth, trim={0 0 0 0},clip]{./figures/tot.png}
	\vspace{-.5em}
	%\captionsetup{skip=3pt}
	\caption{Example \llm diagnosis by tree of thought}
	\label{fig:tot}
	\vspace{-1.25em}
\end{figure}

\section{\llm Diagnosis}
\label{sec:diagnose}

\hi{Tree Search Algorithm using \llm.} To avoid diagnosis failures caused by the incorrect actions (e.g., non-existent API name) derived by \llm, we propose to utilize the {\it tree of thought} strategy that can guide \llm to go back to previous actions if the current action fails. %It significantly increases the likelihood of \llms arriving at reasonable diagnosis results (Section~\ref{sec:diagnose}).

\textit{Step1: Tree Structure Initialization.} We initialize a tree structure, where root node is the diagnosis request (Figure~\ref{fig:tot}). Utility methods are utilized to manipulate the tree structure, and UCT score for node $v$ are computed based on the modifications during planning, i.e., $\text{UCT}(v) = \frac{w(v)}{n(v)} + C \cdot \sqrt{\frac{\ln(N)}{n(v)}}$, where $\frac{\ln(N)}{n(v)}$ denotes the selection frequency and $w(v)$ denotes the success ratio of detecting root causes. Note, the action of $n(v$ fails to call tool API,  $w(v)$ equals -1.

\textit{Step2: Simulate Execution.} This step kickoffs the execution of simulations starting from the root node of the tree. It involves selecting nodes based on specific standard (e.g., detected abnormal metrics). If the criteria for selecting a new node is met, a new node is chosen; otherwise, the node with the highest UCT value is selected. 

\textit{Step3: Existing Node Reflection.} For each node in the path from the root node to the selected node, reflections are generated based on decisions made at previous nodes. For example, we count on \llm to rethink the benefits of analyzing non-resource relevant metrics. If \llm decides the action cannot find any useful information, the UCT value will be reduced and set to that of its parent node. In this way, we can enhance the diagnosis efficiency.

\textit{Step4: Terminal Condition.} If \llm cannot find any more root cause (corresponding to a leaf node) for a threshold time (e.g., five), the algorithm ends and \llm outputs the final analysis based on the detected root causes.

% There are mainly two critical parts in $x'$: (1) instruction to guide \largemodel, and $(ii)$ demonstration examples for \largemodel to simulate. The generated prompts should be validated by the feedback of \largemodel, based on which we can optimize the generator for good \largemodel performance. Furthermore, when we use prompts to interact with \largemodel, we should reduce the interaction latency (e.g., reducing interaction rounds) and cost  (e.g., the input token number of each interaction round) for real applications. 

%The vanilla few-shot prompt learning whereby models are provided with a prompt consisting of several examples for the given task, has been shown to fail when it comes to problems that require complex reasoning. To address this issue, we can  utilize Chain-of-Thought (CoT) prompting. Unlike vanilla few-shot prompt learning, CoT additionally inserts the reasoning trace required to derive the final answer for each example in the prompt. In this way, CoT prompts models to generate their ``thoughts'' on the necessary intermediate steps before arriving at the final answer. CoT has been proven to significantly boost performance on a wide range of tasks, including arithmetic reasoning, commonsense reasoning, and symbolic reasoning.  


%Moreover, when diagnosing security vulnerabilities, AutoGPT combined with Langchain helps \llm to construct security threat scenarios systematically. This approach allows for better analysis of potential attack vectors and enhances database protection. Additionally, leveraging the advanced capabilities of GPT-4 in database diagnosis empowers \llm to understand intricate contexts and make well-informed decisions.


%In the final step of database diagnosis, answers are constructed based on the data obtained from the queries. Various approaches can be employed to present the findings effectively. Observations can be shortened manually or automatically to offer concise insights. Flexible data retention criteria allow retaining valuable information, even if errors occur but are later corrected. For cases where API calls may result in errors, simulating API results provides valuable data for analysis. Additionally, methods like Monte-Carlo Search explore diverse solutions, while converting chain-of-thought into a tree-of-thought approach organizes complex concepts coherently. The combination of AutoGPT and Langchain streamlines tree-of-thought generation. Furthermore, utilizing GPT-4 enhances the language model's accuracy and context awareness, contributing to more accurate and contextually relevant diagnoses. Such techniques facilitate improved problem-solving and make \llm a valuable tool in database diagnosis and maintenance.

%\textit{Answer Construction.} The final step centers on constructing answers based on the data generated by the queries. Various approaches can be adopted, such as shortening observations (manually or automatically) for more concise answers. Additionally, modifying criteria for retaining data enables the retention of information, even if an error occurs but is later corrected. For cases where an API call might result in an error, simulating API results can provide valuable data. Other methods, such as Monte-Carlo Search, converting chain-of-thought into a tree-of-thought approach, employing AutoGPT + Langchain for generating a tree-of-thought, or utilizing GPT-4, can all contribute to the answer construction process.


%When learning to utilize a specific tool, human beings perceive it as an object with particular functions, engaging in a cognitive process to understand its purpose and operation. By observing goal-directed demonstrations and following actions performed by other people, they gradually acquire the necessary knowledge and skills to use the tools effectively. Similarly, this understanding process is crucial for successfully solving tasks with tools. Analogously, a comprehensive understanding of the tools' functionalities is indispensable for enabling the controller to use tools proficiently. The process of tool understanding encompasses grasping what the tool is used for and how to use the tool. \revise{add} %Take the case of a calculator: the controller needs to know that a calculator is intended for arithmetic operations, its input should be numbers and mathematical operators, and its output should be a computed value.


%need to conduct reasonable diagnosis for typical database problems (anomalies). As mentioned above, different rule-based diagnosis, \llms can flexibly understand different diagnosis experience and apply to similar cases. However, there are still several challenges. First, beyond prepared experience, we need to teach \llms to obtain detailed information and available optimization actions by calling external tools ({\it tool learning}). 

\iffalse
\begin{lstlisting}[language=python]
# Few-Shot Prompt
Diagnose the causes of a performance problem and give some optimization suggestions.
First, obtain time period the anomaly and memorize the start and end time of the anomaly.
Second, diagnose the causes of the anomaly.
Third, you need to match each cause with potential solutions cached in the knowledge base.
Finally, list the above diagnosed causes and their matched solutions in easy-to-understand format using bullet points.
================================
# A Demonstration example:
...
\end{lstlisting}

\hi{Tree Search Algorithm using \llm.} With the new extracted optimization rules, they greatly enlarges the candidate plan space, which grows exponentially with the number of optimization rules. Consequently, this increases the expense or computational cost of using \llm in query planning. Therefore, we propose to employ an efficient tree search algorithm to guide the planning procedure of \llm.  Although various methods have been proposed for query optimization~\cite{DBLP:journals/pvldb/MarcusNMZAKPT19,DBLP:conf/sigmod/YangC0MLS22,DBLP:journals/pvldb/ZhouLCF21}, they cannot effectively understand the contextual query information (e.g., query patterns that are potential bottlenecks) and accordingly schedule actions (e.g., calling rules). Thus, we introduce an \llm-based optimizer planning algorithm, which involves five steps.

\textit{Step1: Foundation Model Initialization.} We initialize a tree data structure, where the root node is the origin query. Utility methods are utilized to manipulate the tree structure, and UCT score for node $v$ are computed based on the modifications during planning, i.e., $\text{UCT}(v) = \frac{w(v)}{n(v)} + C \cdot \sqrt{\frac{\ln(N)}{n(v)}}$, where $\frac{\ln(N)}{n(v)}$ denotes the selection frequency and $w(v)$ denotes the cost reduction over origin query.

\textit{Step2: Simulate Execution.} This step kickoffs the execution of simulations starting from the root node of the tree. It involves selecting nodes based on specific standard (e.g., lower estimated cost than all the existing nodes). If the criteria for selecting a new node is met, a new node is chosen; otherwise, the node with the highest UCT value~\cite{DBLP:journals/pvldb/ZhouLCF21} is selected. 

\textit{Step3: Existing Node Reflection.} For each node in the path from the root node to the selected node, reflections are generated based on decisions made at previous nodes. For example, we count on \llm to rethink the benefits of applying {\it AggregateFilterTranspose} rule in $N_2$. 
If \llm decides the rule actually cannot reduce the computation complexity, the UCT value of $N_2$ will be reduced and set to that of its parent node. In this way, we can reduce the bias caused by cost estimation errors and guide query planning more robustly.

\textit{Step4: Terminal Node Selection} In this step, a voting process is conducted among the terminal nodes to determine the most appropriate node(s) for the given optimization task. For example, although $N_4$ and $N_5$ share similar execution costs, $N_4$ is selected as the terminal node, because the query pattern of $N_4$ is more similar to the origin query and may be less likely to produce wrong execution results \revise{replace with a better example}.
\fi


\iffalse
\begin{figure*}[!t]
	\centering
	\includegraphics[width=\linewidth]{./figures/result_index.pdf}
	\vspace{-1em}
	\captionsetup{skip=0pt}
	\caption{Index optimization results.}
	\label{fig:modelFig}
	\vspace{-.5em}
\end{figure*}
\fi


==> 05-optimization.tex <==
%!TEX root = ../main.tex
\section{Intra-operator Optimizations}
\label{sec:intra-optimization}

The optimization of each operator in \sys consists of a sequence of optimizer modules, namely cacher, validator, simulator, ensembler, and adaptor.

\todo{ordering: first introduction, then examples}

\subsection{Cacher}
\label{sec:cacher}

The cacher applies mainly for the direct querying of LLMs, as it is common to encounter numerous highly similar or even identical inquiries in the data. For a specific LLM, it provides similar or identical results for these inquiries, leading to inefficiencies in terms of repeated LLM calls. To address this issue~\cite{gpt-cache}, we introduced a cacher that leverages a small, frozen language model $\mathcal C$ to index and store the results of similar inquiries.

Consider the scenario of a web-content topic classification task. LLMs have demonstrated a remarkable capacity to accurately identify the subject matter of a given web content. As such, they could be employed as a potent instrument to directly address this challenge. However, to further improve their efficiency, LLMs can be utilized in an alternative manner - as annotators that identify and extract representative samples for each topic. By adopting this approach, the classification of new content can often be achieved by simply comparing it to the most similar examples, thereby reducing the need to rely on LLMs only for challenging cases. Furthermore, this approach ensured consistency in relation to the copious recurring content on the internet, which was showcased via replication, excerpts, and references. In \sys, the responsibility of storing these samples and recommending them based on their similarity lies with the cacher component.

Specifically, the cacher deploys $\mathcal C$ locally and creates an index for each input question $Q$ of the LLM using the vector output $\mathcal C(Q)$. The model is frozen so that the vector index is not changed. As the parameters of $\mathcal C$ are initialized by a pre-trained language model, $\mathcal C(Q)$ could provide a meaningful index without fine-tuning. In the aforementioned web-content topic classification example, we can simply cache $\mathcal C(\text{topic-classification} \oplus C)$ where $C$ denotes the web content and $\oplus$ denotes string concatenation with separators. For a more complicated example, to differentiate names from non-name noun phrases in the case of name extraction task, the cacher could use $\mathcal C(\text{name-extraction}\oplus T \oplus NP)$ to establish an index, where $T$ is the full-text passage and $NP$ is the proposed noun-phrase.

When a new inquiry is received, the cacher retrieves the top-$K$ most similar inquiries from the index to assist in processing the current inquiry. For classification problems, the cacher can directly obtain the result of the new inquiry through a majority ensemble, eliminating the need to query the LLM completely. For more open-ended questions, the top-$K$ similar inquiries can be integrated into prompts to the LLM, which can help improve the LLM's accuracy.

It is important to note that the cacher does not fine-tune the small language model $\mathcal C$. This is to ensure that the obtained vector $\mathcal C(Q)$ remains consistent for a fixed input $Q$ and can be stored. This guarantees the availability of conventional vector-based indexing techniques such as FAISS~\cite{faiss}, which allows the efficient retrieval of similar inquiries. If fine-tuning is required, a simulator (Sec.~\ref{sec:simulator}) may be more appropriate for optimizing this task. While it is possible to periodically fine-tune $\mathcal C$ to achieve more accurate semantic indexing, we do not recommend it as other optimizer modules such as a simulator can cover this functionality. The cacher primarily addresses efficiency and instant re-use.

Overall, the cacher is a practical approach to improving the efficiency and accuracy of LLMs in question-answering tasks. By leveraging the similarity between inquiries, we can reduce the number of repeated LLM calls and enhance the accuracy of the model.

\subsection{Validator}
\label{sec:validator}

Consider the scenario of tokenization, a seemingly simple task that can be implemented with just a few lines of code. However, complexities arise when dealing with letter cases, dates, punctuation, special characters, foreign languages, and so on. In specific situations, the behavior of a tokenization process must be clearly defined through examples and verified against these examples. In fact, for any operators, it is essential to guarantee their accurate and effective performance in executing their intended functions. This necessitates adherence to predefined specifications and requirements while minimizing errors and deviations from expected outcomes. To attain this degree of reliability and precision, \sys proposes introducing a validator that rigorously tests and debugs all operators, regardless of whether they are implemented by LLMs, generated by LLM codes, or manually written codes, among others.

The validator is versatile and can be used on any operator. Its primary function is to facilitate automatic testing and debugging of operators. Recent research~\cite{react,reflexion} on LLM interaction has highlighted the importance of providing error feedback to LLMs and explored the potential of utilizing LLMs to assist in delivering such feedback. However, the current state of research on LLM error correction remains in its early stages: the experience in error fixing, which has been refined through trial and error within a single data point, is difficult to generalize to new instances. Furthermore, a formal procedure for rectifying errors has yet to be established. In the \sys system, we have refined the error feedback and suggestion involving LLMs, developed a complete procedure for generic error fixing, and broadened their scope to include code generation and code debugging.

% \lei{In general it is NOT clear how validator works.}

The automatic validator we propose consists of the following main steps:

\todo{add illustration figure}

\begin{compactitem}
    \item {\textbf{Verifier}}: The verifier necessitates that operators supply examples during the operator definition process. It assesses the accuracy of the operator's execution and confirms if the results on the provided examples align with the expected outcomes. The verifier can be a standard verifier, which typically demands the operator's output results to match the provided examples exactly, or a custom verifier, which can be acquired by integrating a standard verifier with a custom operator that offers a more adaptable definition of output accuracy. Pre-existing operators in the \sys system are accompanied by their own examples, and in data preprocessing, the \sys system automatically extracts and generates examples (Sec.~\ref{sec:generation}).
    
    \item {\textbf{Advisor}}: The advisor module serves a function akin to the Reflection LLM in Reflexion~\cite{reflexion}. It proposes modifications for prompts (for direct queries) and code (for code generation/debugging) based on historical prompts, historical code/queries, examples, example results, and error types. The historical prompts and code are facilitated by the code generation operator, as mentioned earlier. Meanwhile, the verifier's execution result determines the examples, example results, and error types. The LLM receives the combined input and generates a plan to fix the code, either by reverting to a previous version or creating a new one. If the LLM suggests generating a new code version, it is asked to further provide high-level insights into the error's cause and potential generic fixes. These suggestions can be used for user-facing interactions or as reference points for subsequent validation steps. By default, the advisor module uses an LLM to produce suggestions, but manual suggestions can be employed as an alternative when validation repeatedly fails.
    
    \item {\textbf{Code Validator}}: The code validator in the automatic validator is only applicable to operators with code attached. It modifies the code based on various inputs, including historical prompts, historical code, examples, example results, and error types. Most of these inputs are also used by its predecessor, the advisor. Additionally, the code validator incorporates suggestions derived from the advisor. The LLM processes the combined information to directly generate a new code version based on the advisor's suggestions. After modification, the automatic validator starts a new validation round and re-evaluates the examples using the verifier and advisor, completing the overall validation mechanism.
    
    \item {\textbf{Prompt Validator}}: The prompt validator within the automatic validation system is primarily designed for LLM queries. It adjusts prompts by considering historical prompts, code, examples, example results, error types, and suggestions. Notably, it can function as a fallback mechanism for the code validator when validation repeatedly fails. In other words, if the advisor and code validator cannot generate code that is suitable for most or all examples after several validation rounds, the prompt validator can intervene to modify the initial prompt in the code generation configuration. This process generates a new version tree of codes, potentially reducing the need for human intervention in the advisor.
\end{compactitem}

In summary, the validator we propose is a powerful tool for testing and debugging operators. It is compatible with any operator. Its sub-components: verifier, advisor, code validator, and prompt validator, work together to provide comprehensive feedback and suggestions for improving the operator's performance.

\todo{add example tokenization}

\todo{elaborate}

\subsection{Simulator}
\label{sec:simulator}

The simulator is suitable for any operator with high execution costs. Unlike the cacher with static vector indexing, the simulator introduces a more complex encoding process that provides better flexibility and accuracy.

Consider the scenario of entity resolution. As previously mentioned in the introduction of the cacher (Section \ref{sec:cacher}), end-to-end LLMs may be capable of performing these tasks. However, they might not be as efficient as a localized solution. In the context of entity resolution, directly deploying a cacher to leverage historical queries may not be effective. This ineffectiveness can be attributed to several factors. First, the similarity measure used to determine whether two entities are identical is typically scenario-specific and unsuitable for a single frozen local model. Second, entity resolution places greater emphasis on the differences between query entities rather than their similarities, resulting in numerous potential false positives when using a naive similarity-based approach. Consequently, a tunable and adaptive measure is called for to localize the process of entity resolution effectively.

As mentioned above, any operator can be viewed as a black-box function $f: X \to Y$. The simulator continuously keeps track of the $(X,Y)$ obtained during online operation after the deployment of the data science application. When a pre-defined trigger is met (e.g., every $5000$ accumulated data records), the simulator re-trains a local model $\mathcal S_f$ to imitate the operator's behavior. The local model can then be used to replace the original operator when the accuracy or confidence exceeds a pre-defined threshold. It is important to note that the accuracy here does not represent the accuracy of the actual function to the ground truth, but rather the degree of agreement with the original operator's execution results. Using the local model $\mathcal S_f$ instead of the original operator can improve efficiency if the execution cost of the original operator is higher than that of the local model.

% \lei{Given a task, who and how to decide which model to use? No parameter tuning is needed?}

\todo{tuned large model add another section: details about LoRA}

The \sys system applies different types of local models depending on the input and output $(X,Y)$. Available choices are as follows:
\begin{compactitem}
    \item {\textbf{Small Language Model}}: A locally deployed sequence-to-sequence (Seq2Seq) model is the most common type of local model for simulating any serializable input $X$ and output $Y$. It is trained on self-supervised learning tasks such as autoregression on all collected data $(X \oplus Y)$ and can be used for conditional generation at inference time given $X$. Note that the encoder of the small language model can also be used for other purposes such as generating a vector representation of $X$ (more flexible and fine-tunable than the cacher, but not suitable for indexing regarding efficiency). Therefore, this tunable small language model can be used with shared parameters across multiple related modules.
    
    \item {\textbf{Tuned Large Model}}: The emergence of open-source LLMs such as LLaMA~\cite{llama} has made it possible to locally fine-tune LLMs. However, fine-tuning LLMs is an expensive process. Recent research has developed delta-tuning techniques such as LoRA~\cite{lora} to tune local LLMs. The LoRA technique introduces a low-rank matrix added to the original model parameters, which is updated instead of the original parameters during the tuning process. As the matrix is assumed to be low-rank, it can be represented by a decomposition matrix and a dimension-expansion matrix, both of which are much smaller than the original parameter matrix. This method can significantly reduce the number of parameters that need to be updated in tuning large language models and is therefore widely used. It is worth noting that the LoRA technique can not only be used for tuning LLMs but has also been applied in vision models~\cite{sd}. The simulator based on fine-tuned large models provides potential support for optimizing multi-modal data science applications within the \sys system.
    
    \item {\textbf{Classification Model}}: For cases where $Y$ has only a small number of categories, a classification head with an arbitrary encoder structure can be used as a local model for supervised learning. A classification model usually achieves better results than a universal sequence-to-sequence model. Furthermore, when instructed by the user, \sys simulator could cluster similar operator outputs to enable the usage of a classification model.
    
    \item {\textbf{Regression Model}}: For cases where $Y$ mainly contains numerical outputs, a regression head with an arbitrary encoder structure can be used as a local model for supervised learning. However, learning for regression problems with unstable numerical ranges can be difficult and is not recommended.
    
    \item {\textbf{Conventional Model}}: In data science, it is common for both $X$ and $Y$ to mainly consist of numerical or categorical features. More traditional machine learning methods such as linear regression, polynomial regression, elastic net regression, support vector machines, decision trees, XGBoost, etc. These methods have stronger interpretability but lower flexibility. Therefore, conventional models are not automatically applied by the \sys system and mainly rely on users with programming experience to choose.
\end{compactitem}

In practice, simulators operate almost autonomously: \sys utilizes a classification model for outputs with limited categorical values and a regression model for numerical outputs. For other scenarios, the small language model acts as a default option, unless the user specifically selects a tuned large model or a traditional model. By default, simulators apply only to direct query operators, unless stated otherwise, since generated or manual code is more efficient than machine learning models in most cases.

Apart from the local model choice and implementation, another important issue worth paying attention to is the control logic to determine when to substitute the original operator with the local model and when to stick to the original operator. The most straightforward strategy is to set a global threshold (e.g., $90\%$): whenever the accuracy of the local model is higher than the threshold, the local model completely bypasses the execution of the original operator.

However, various data points within the same task often exhibit differing levels of complexity. For instance, in named entity extraction, as previously mentioned, "Lincoln" is an ambiguous term that could represent multiple entities, whereas "Emily" is almost certainly a human name. Another example can be found in entity resolution; while most entities can be deduced through traditional similarity measures, identifying that "IBM" and "Big Blue" represent the same company is challenging without employing the common sense embedded in LLMs\footnote{"Big Blue" is the nickname of IBM, named after its blue logo.}. Consequently, a more efficient replacement method should rely on the confidence of the local model concerning the relevant data points.

\todo{as an independent section}

Most local models could obtain confidence indicators as a byproduct of their execution. For example, for classification models, the probability of the class with the highest predicted probability can be regarded as a confidence indicator: the closer the probability of the class with the highest predicted probability is to $1$, the higher the prediction confidence. For language models, the perplexity of the generated text can also be regarded as a confidence indicator: the lower the perplexity, the higher the prediction confidence. However, it should be emphasized that the confidence indicators provided by the model itself are empirical and cannot provide theoretical guarantees for the accuracy of the model. A non-robust model may output incorrect predictions with high confidence. Another commonly used confidence criterion is achieved through ensembles, for example: training multiple models with different initializations, and the number of models obtaining the majority classification on a data point can be regarded as a confidence indicator.

\todo{Technique: induce confidence from LLM API}

It is important to highlight that simulators can not only enhance the execution efficiency of operators but also increase their accuracy. In a teacher-student paradigm, it is commonly believed that the performance of a student model (in this case, the local model) is limited by its teacher model (in this case, the original operator). However, research~\cite{bootstrapping,bootstrapping2,distillation,toolformer} has demonstrated that a student model, obtained through self-training on the filtered output of the teacher model, may outperform the teacher model, a phenomenon known as bootstrapping. This occurs because filtering the teacher model's output and retaining only high-confidence data results in slightly higher-quality training data for the student model compared to the raw data used by the teacher model. Furthermore, since the local model can continuously learn the real data distribution after deployment by the data custodian and adapt to manually corrected erroneous labels, it can progressively surpass the original static operator over time.

\subsection{Ensembler}
\label{sec:ensembler}

In the majority of data science applications with verifiable outputs, such as classification problems (e.g., entity resolution and topic classification) with clearly defined ground truths, employing an ensemble of multiple models can potentially lead to superior outcomes compared to relying on a single model.

The role of the ensembler involves generating various diverse models and pinpointing the most effective ones with the assistance of validator modules. Owing to the substantial disparity in computational complexity between direct query and code generation, these methods are typically ensembled independently.

Regarding the integration of LLMs into the ensemble, in the context of the direct query, the ensembler promotes diversity in the initial prompt and the prompt validator. More specifically, the LLM is responsible for rephrasing the prompts to produce alternative results. In the context of code generation, the ensembler focuses on the initial prompt and code validator, requiring the LLM to implement the provided function in distinct ways. In addition to employing LLMs, operators with verifiers also facilitate diversification based on the chosen failure cases.

\todo{pseudo-code on genetic algorithm}

The ensemble method incorporates the majority voting ensemble as its simplest yet most adaptable technique. Additionally, using an accuracy-weighted voting strategy provides a more versatile solution with the ability to exclude low-accuracy candidates. Specifically, a predetermined number $M$ of prompt and code variations are generated through LLM-advised prompts or randomly selected failure cases from the verifiers during each iteration. The top $m < M$ variations are preserved and employed to generate the next iteration of variations. This method is akin to the genetic algorithm, wherein variants are created, assessed, chosen, and mutated. In addition to evaluation and selection based on a fixed set of examples provided by the operator, it is feasible to use data generated by LLMs (Sec.~\ref{sec:generation}) or data annotated (Sec.~\ref{sec:annotation}) post-deployment to further enhance the ensemble process. Beyond accuracy as a criterion, it is also possible to employ a confidence indicator as a dynamic voting weight, as suggested in the simulator section (Sec.~\ref{sec:simulator}).

In most cases, a standard ensembler employed for classification tasks does not introduce additional complexity beyond a minor constant, as the aggregation strategy is straightforward and the ensembled variations exhibit comparable computational complexity levels. However, when striving for improved performance and efficiency is not a limiting factor, employing an LLM ensemble method becomes a viable option. This technique treats the individual outputs as alternatives or components presented in the prompt and the LLM is asked to select a single option or construct more complex responses based on the provided components. Moreover, the ensembler is allowed to create ensembles containing methods of different computational complexity if and when explicitly required.

\todo{rename}
\subsection{Adaptor}
\label{sec:adaptor}

The adaptor in \sys typically serves as an interface that enables the LLMs to access local data and existing data science tools, thereby bridging the gap between these resources and the LLMs' capabilities.

Consider the scenario of NL2SQL, which involves converting natural language queries into SQL queries for a specific database. On the one hand, it is generally both insecure and inefficient to provide the entire database as input to the LLM. On the other hand, supplying only the table schema could restrict the LLM's ability to generate SQL queries with correct predicate values. To address similar challenges in presenting local data and local tools to LLMs, a unified and enhanced approach is necessary.

The adaptors comprise the following main types:
\begin{compactitem}
\item {\textbf{Custom Operators}}: Utilizing a modularized approach, both built-in and user-defined operators in \sys can act as building blocks for new user-defined operators. Specifically, for any operator $f:X \to Y$ defined within the \sys system, the adaptor generates a description $(d_f, d_X, d_Y)$ about the operator, input, and output to be provided to LLMs, as well as an API for $r_f$ in a specified programming language, such as Python. As a result, the adaptor can be invoked by the LLMs through interaction or by code generated by the LLMs.

\item {\textbf{Custom Data Science Tools}}: Given the diverse nature of data science applications, it is often more efficient and effective to incorporate existing data science tools as a single step within a comprehensive data science application. For instance, when analyzing periodic time series data, providing FFT as an available tool can streamline code generation by LLMs and enhance their ability to develop a more effective data science application. For widely used public data science tools, LLMs can already leverage their power as they are present in the code contained in the pre-training corpora. However, for private packages, users can provide the description $(d_f, d_X, d_Y)$ about the tools, as \sys does for built-in operators. Alternatively, users can supply use cases or documentation, which can then be fed to the LLMs to automatically generate the description $(d_f, d_X, d_Y)$. While the latter approach is more convenient, its effectiveness is not guaranteed.

\item {\textbf{Local Data}}: One of the most vital roles of the adaptor is to enable access to local data. Local data in data science applications can be extensive, private, and organized in various ways. As a result, the interface for accessing local data should be interactive, privacy-preserving, and unified. \sys provides built-in adaptors of this type, including Long Text Adaptors, Knowledge Graph Adaptors, Search Engine Adaptors, SQL Adaptors, etc., which serve as intermediate components between the LLMs and users. Users can set up any local server to respond to queries posted by the adaptors, and the adaptors should manage the process of handling queries and sending responses to the LLMs. Privacy is preserved under the control of the local server, while interaction and unification are achieved by the adaptors' implementation. More details about how adaptors efficiently intervene in the process of data access are discussed in Section \ref{sec:pre-processing}.

\item {\textbf{Workspace}}: The concept of utilizing memory to enhance the capabilities of LLMs has been a topic of interest in recent works~\cite{autogpt,langchain,recurrentgpt,scm}. These studies primarily treat memory as preserved textual prompts within a single dialogue, which can limit the scope of information retention and retrieval. In contrast, \sys introduces a more advanced and flexible workspace adaptor, which allows for memory storage in the local environment, thereby expanding the LLMs' capacity to manage and access information. Specifically, the workspace adaptor enables LLMs to store information as key-value pairs, which can be retrieved later as needed. \sys provides key-based value retrieval, similar key retrieval, and key listing to retrieve the stored information. Key-based value retrieval allows LLMs to access specific information directly by referencing the associated key, while similar key retrieval enables the identification and retrieval of related information based on key similarity. Additionally, key listing provides an overview of all existing keys in the local storage, facilitating easier navigation and management of stored information. By implementing the workspace adaptor, \sys allows LLMs to update and maintain information persistently even after the online deployment of the data science application. This enhanced memory management capability not only improves the efficiency and effectiveness of LLMs but also enables them to handle more complex tasks and develop more robust data science applications.
\end{compactitem}

The adaptors, which enable the integration of pre-defined operators, data science tools, and access to local data and storage, serve as crucial components in the \sys system for enhancing the efficiency of these operators.

\section{Inter-operator Optimizations}
\label{sec:inter-optimization}

Inter-operator optimization offers a substantial potential for enhancement in data science applications, going beyond the optimization of individual operators. The main goal of this optimization is to improve the overall planning and coordination of operators while preserving the modularity of treating each operator as a separate black box. This approach mainly concentrates on the organization and integration of operators. By broadening the optimization scope beyond a single operator, a more holistic and efficient strategy can be implemented for a wide array of prevalent data science applications.

To optimize a diverse data science application, it is crucial to focus on the bottleneck components, as each component may display different levels of computational complexity. The \sys system classifies operators based on their computational complexities, which consist of:

\begin{compactitem}
    \item {\textbf{Massive}}: This complexity level involves an operator that is considerably more costly than an LLM API call, typically necessitating the processing of a vast amount of local data to answer a single query.
    \item {\textbf{Significant}}: This level of complexity is analogous to an LLM API call.
    \item {\textbf{Moderate}}: Often representing the execution of a local machine learning-based solution or a data science tool. This complexity level is faster than an LLM API call but slower than straightforward data processing.
    \item {\textbf{Low}}: Basic processing of data. This complexity level is more or less comparable to scanning the data record.
    \item {\textbf{Minimal}}: Generally sub-linear. This level of complexity enables answering a query without processing the entire data required by the query.
\end{compactitem}

The inter-operator optimizations in \sys primarily involve substituting high-category operators with lower-category operators and absorbing lower-category operators into higher-category ones.

By focusing on the optimization of bottleneck components in a data science application, the system can effectively handle the diverse computational complexities of each component, leading to improved overall performance.

\todo{add section: cite volcano, pipeline execution scheme}

\subsection{Predicate Pushdown}
\label{sec:predicate-pushdown}

In numerous data science applications, it is often anticipated that data analysis will be conducted on a specific subset of the available data. As a result, identifying and isolating this filtered data at the earliest opportunity could lead to the elimination of the need for running computationally heavy operators thereby significantly improving computational efficiency.

In \sys, a special type of operator, the filter operator is designated for reducing the number of data records based on a condition, which could be either a simple expression or more general, the execution result of a custom operator. Consider describing the dependency of operators as a tree structure, the objective of predicate pushdown is to move the filter operator downwards as close to the raw data source as possible, most importantly before the execution of operators with high computation complexity.

The most direct and comprehensive approach involves employing a learning-based method to predict the filter predicate. This concept has previously been introduced in the simulator section (Sec.~\ref{sec:simulator}), where a local model is trained on deployed data to replicate the execution outcome. In this context, a local model is developed for each filter operator that has at least one massive, significant, or moderate operator preceding it in the pipeline. The purpose of this model is to predict whether the data should be discarded before reaching the computationally expensive operators.

In more complex cases involving predicate decomposition, the \sys system conducts a greedy search for each subtree with the filter operator as the root, aiming to identify the maximum block that can be bypassed accurately. Initially, only the filter operator is included in the subtree to be bypassed. After deployment, \sys collects data online and maintains a record of the average running time for each operator. Utilizing these statistics, the \sys system attempts to dynamically expand the tree. During periodic local model training, the system evaluates whether adding another layer of children or incorporating a specific child with a high average running time to the current subtree could produce a local model that meets the threshold for filtering out data.

\todo{add illustration figure}

This approach addresses the potential pushdown of placing filter predicates beneath moderate-complexity operators. The remaining need for further pushdown of predicates involves replacing low-complexity filters with minimal-complexity filters. Given the diverse nature of data science applications, such filters should be managed in conjunction with the \texttt{LOAD\_DATA} operator (Sec.~\ref{sec:pre-processing}), guided by human input and converted by the \sys system.

\subsection{Operator Compression}
\label{sec:operator-compression}

As opposed to the predicate pushdown in \sys, which typically replaces groups of high-complexity operators with a single moderate complexity operator (a learning-based local model), the operator compression in \sys mainly absorbs low-complexity operators with the high-complexity operators above and beneath it in the execution pipeline.

Specifically, for any operator that does not require a large amount of local data (non-massive operators), using an LLM query as a black-box simulator is viable. In general, an LLM query is highly resource-intensive, rendering such a simulation unworthy. However, when a significant-complexity operator is already present in the pipeline, it becomes feasible to employ an LLM to mimic an operator with similar computational complexity while simultaneously extending it to its related predecessors and successors, thereby marginally enhancing the overall running time.

\section{Data Processing}
\label{sec:processing}

\todo{split data processing into other sections?}

In the rapidly expanding field of data science, researchers often find themselves dedicating a substantial portion of their time and effort to preprocessing the heterogeneous data they encounter. The preprocessing stage, therefore, serves as a crucial step in transforming raw data into a clean, well-structured format for further analysis. With the help of LLMs, \sys has developed multiple methods in improving the processing and understanding of user-specified local data.

\subsection{Automatic Preprocessing}
\label{sec:pre-processing}

Firstly, when assuming that a portion or all of the local data is homogeneous and in a serializable format, the system can directly utilize the code generation operator to specify a \texttt{LOAD\_DATA} operator. For more complex cases, the \texttt{LOAD\_DATA} operator can be enhanced by validators (Sec.~\ref{sec:validator}), particularly the advisors, which serve as another LLM capable of explaining the data format and consequently provide a natural language guide for the code generation of the \texttt{LOAD\_DATA} operator.

However, in numerous instances, the potential input data size surpasses the context length of most existing LLMs. Moreover, considering efficiency and security concerns, local data should be presented to the LLM using a specified protocol. In the \sys system, a data processing protocol necessitates users to establish a local server with designated APIs that can be accessed by the LLM via adaptors, acting as the client. Defining such APIs may be an unnecessary task for simple data science applications; therefore, the system has established several protocols for common data science scenarios.

\subsubsection{Processing of Long Textual Data}
\label{sec:long-text}

\subsubsection{Processing of Knowledge Graphs}
\label{sec:knowledge-graphs}

\subsubsection{Data as Local Search Engine}
\label{sec:search-engine}

\subsubsection{Data as Structured Database}
\label{sec:sql}

\todo{}

\subsection{Generation}
\label{sec:generation}

\todo{}

\subsection{Annotation}
\label{sec:annotation}

\todo{}



==> 05-update.tex <==
%!TEX root = ../main.tex


\section{Collaborative Diagnosis For Complex Cases}
\label{sec:collaborate}

 A single \llm may be limited in its ability to fully resolve a problem (e.g., stuck in initial steps). Collaborative diagnosis involves the utilization of multiple \llms to collectively address complex cases by leveraging their unique role capabilities. This section introduces the communicative framework for database diagnosis~\cite{agentverse,qian2023communicative}.

\begin{compactitem}
	\item
	\begin{sloppypar}
	\bfit{Agents.} In the communicative framework, agents can be undertaken by human beings or \llms. Humans can provide \llm agents with scenario requirements (e.g., business changes over the incoming period) and prior knowledge (e.g., historical anomalies). On the other hand, each \llm agent is dedicated to a distinct domain of functions. For example, we include three \llm agents in the initial implementation: (1) Chief DBA is responsible for collaboratively diagnosing and detecting root causes with other agents; (2) CPU Agent is specialized in CPU usage analysis and diagnosis, and (3) Memory Agent focuses on memory usage analysis and diagnosis. Each \llm agent can automatically invoke tool APIs to retrieve database statistics, extract external knowledge, and conduction optimizations. For instance, CPU Agent utilizes the monitoring tool {\it Prometheus} to check CPU usage metrics within specific time periods, and determine the root causes of high CPU usage by matching with extracted experience (Section~\ref{sec:prepare}). Note, if CPU/memory agents cannot report useful analysis, Chief DBA is responsible to detect other potential problems, such as those on the application side.
	\end{sloppypar}	

	\vspace{.5em}

	\item
	\bfit{Environment Settings.} We need to set a series of principles for the agents to efficiently communicate, such as {\it (1) Chat Order:} To avoid the mutual negative influence, we only allow one \llm agent to ``speak'' (i.e., appending the analysis results to the chat records to let other agents know) at a time. To ensure flexible chat (e.g., if an agent cannot detect anything useful, it should not speak), we rely on Chief DBA to decide which agent to speak in each iteration (diagnosis scheduling); {\it (2) Visibility:} By default, we assume the analysis results of agents can be seen by each other, i.e., within the same chat records. In the future, we can split agents into different groups, where each group is in charge of different database clusters/instances and they do not share the chat records; {\it (3) Selector} is vital to filter invalid analysis that may mislead the diagnosis directions; {\it (4) Updater} works to update agent memory based on the historical records.


\sbox{\blackball}{\tikz \fill[red] (0,0) circle (.5ex);}
\sbox{\greenball}{\tikz \fill[codegreen] (0,0) circle (.5ex);}


\begin{table*}[htbp]
	\centering
	\caption{Diagnosis performance of single root causes (\usebox{\blackball} : legal diagnosis results; \usebox{\greenball} : accurate diagnosis results).}
	\label{tbl:results}
	\vspace{-.25em}
	\begin{tabulary}{\linewidth}{|c|l|L|l|l|}
		\hline
		Type & \textbf{Root Cause} & \textbf{Description} & \textbf{LLM+Metrics} & \textbf{\oursys} \\
		\hline
		{Data Insert} & INSERT\_LARGE\_DATA & Long execution time for large data insertions & \usebox{\blackball} & \usebox{\blackball} \usebox{\greenball} \\
		\hline
		\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Slow\\ Query\end{tabular}} & FETCH\_LARGE\_DATA & Fetching of large data volumes & \usebox{\blackball} \usebox{\greenball} & \usebox{\blackball} \usebox{\greenball} \\
		\cline{2-5}
		& REDUNDANT\_INDEX & Unnecessary and redundant indexes in tables & \usebox{\blackball} & \usebox{\blackball} \\
		\cline{2-5}
		& LACK\_STATISTIC\_INFO & Outdated statistical info affecting execution plan & \usebox{\blackball} & \usebox{\blackball} \usebox{\greenball} \\
		\cline{2-5}
		& MISSING\_INDEXES & Missing indexes causing performance issues & \usebox{\blackball} \usebox{\greenball} & \usebox{\blackball} \usebox{\greenball} \\
		\cline{2-5}
		& POOR\_JOIN\_PERFORMANCE & Poor performance of Join operators & \usebox{\blackball} & \usebox{\blackball} \usebox{\greenball} \\
		\cline{2-5}
		& CORRELATED\_SUBQUERY & Non-promotable subqueries in SQL & \usebox{\blackball} & \usebox{\blackball} \usebox{\greenball} \\
		\hline
		\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Concurrent\\ Transaction\end{tabular}} & LOCK\_CONTENTION & Lock contention issues & \usebox{\blackball} & \usebox{\blackball} \\
		\cline{2-5}
		& WORKLOAD\_CONTENTION & Workload concentration affecting SQL execution & \usebox{\blackball} \usebox{\greenball} & \usebox{\blackball} \usebox{\greenball} \\
		\cline{2-5}
		& CPU\_CONTENTION & Severe external CPU resource contention & \usebox{\blackball} \usebox{\greenball}  & \usebox{\blackball} \usebox{\greenball} \\
		\cline{2-5}
		& IO\_CONTENTION & IO resource contention affecting SQL performance & \usebox{\blackball} & \usebox{\blackball} \usebox{\greenball} \\
		\hline
	\end{tabulary}
	%\vspace{-.5em}
\end{table*}

	\vspace{.5em}
		
	\item
	\bfit{Chat Summary .} For a complex database problem, it requires agents dozens of iterations to give in-depth analysis, leading to extremely long chat records. Thus, it is vital to effectively summarize the critical information from chat records without exceeding the maximal length of \llm prompts. To the end, we progressively summarize the lines of a record used with tools, including inputs for certain tools and the results returned by these tools. Based on the current summary, it extracts the goals intended to be solved with each call to the tool, and forms a new summary, e.g.,
\end{compactitem}




\begin{tcolorbox}[enhanced,sharp corners,
	width={8.5cm},
	colback=white,
	borderline={0.3mm}{0.3mm}{white},
	boxsep=-.5mm]
    {\bf [Current summary]}\\
    - I know the start and end time of the anomaly.
    
    {\bf [New Record]}\\
    Thought: Now that I have the start and end time of the anomaly, I need to diagnose the causes of the anomaly\\
    Action: is\_abnormal\_metric\\
    Action Input: \{``start\_time'': 1684600070, ``end\_time'': 1684600074, ``metric\_name'': ``cpu\_usage''\}\\
    Observation: ``The metric is abnormal''
    
    {\bf [New summary]}\\
    - I know the start and end time of the anomaly.\\
    - {\it {\color{codegreen}I searched for is\_abnormal\_metric, and I now know that the CPU usage is abnormal.}}
\end{tcolorbox}


With this communicative framework and well-defined communication principles, the collaborative diagnosis process among human and \llm agents becomes more efficient (e.g., parallel diagnosis) and effective (e.g., chat records could trigger investigating of in-depth metric observation and root cause analysis). %And we will showcase the importance of communicative \llms over single \llm in the initial experiments.

%The ability to work together, exchange insights, and collectively arrive at more robust solutions greatly enhances the overall diagnostic capabilities of the system.





==> 06-experiment.tex <==
%!TEX root = ../main.tex




\section{Preliminary EXPERIMENT RESULTS}
\label{sec:experiments}

\vspace{.5em}

\hi{Demonstration.} As illustrated in Figure~\ref{fig:demo}, {\it Chief DBA} monitors the status of the database to detect anomalies. Upon recognizing a new anomaly, {\it Chief DBA} notifies both the {\it Memory Agent} and {\it CPU Agent}. These agents independently assess the potential root causes and communicate their findings  (the root causes and recommended solutions) to the \textit{Chief DBA}. Subsequently, the \textit{Chief DBA} consolidates the diagnostic results for the user's convenience. In initial iterations, these agents generally gather limited information, and so they will continue for multiple iterations until the conclusion of {\it Chief DBA} is nearly certain or no further valuable information can be obtained. Additionally, during the diagnosis, users have the option to participate by offering instructions and feedback, such as verifying the effectiveness of a proposed optimization solution.


\begin{figure}[!t]
	\vspace{.5em}
	\centering
	\includegraphics[width=1.05\linewidth, trim={0 7.2cm 0 0},clip]{./figures/demo.png}
	\vspace{-.5em}
	%\captionsetup{skip=0pt}
	\caption{A basic demonstration of \oursys.}
	\label{fig:demo}
	\vspace{-.1em}
\end{figure}


\hi{Diagnosis Performance Comparison.} We compare the performance of \oursys against a baseline, namely \texttt{llm+Metrics}. Both of the two methods are deployed with the OpenAI model GPT-4~\cite{openai} alongside metrics and views from PostgreSQL and Prometheus. The evaluation focuses on basic single-cause problems as detailed in Table~\ref{tbl:results}. Besides, we also offer a multi-cause diagnosis example presented in the \emph{Appendix-B}.

Preliminary results indicate that {\it \llm+Metrics} and \oursys can achieve a high \emph{legality rate} (producing valid responses to specific database issues). However, it is a ``dangerous behavior'' for  {\it \llm+Metrics}, which actually has very low {\it success rate (infrequent provision of the correct causes)}. In contrast, \oursys achieves both high legal rate and success rate. The reasons are three-fold.

First, {\it \llm+Metrics} conducts very basic reasoning and often misses key causes. For example,  for the {\it INSERT\_LARGE\_DATA} case, {\it \llm+Metrics} only finds ``high number of running processes'' with the {\it node\_procs\_running} metric, and stops early. In contrast, \oursys not only finds the high concurrency problem, but analyze the operation statistics in the database process and identifies {\it ``high memory usage due to heavy use of UPDATE and INSERT operations on xxx tables''} by looking up the {\it pg\_stat\_statements} view.

\begin{sloppypar}
Second, {\it \llm+Metrics} often ``makes up'' reasons without substantial knowledge evidence. For example, for the {\it CORRELATED\_SUBQUERY} case, {\it \llm+Metrics} observes SORT operations in logged queries, and incorrectly attributes the cause to ``frequent reading and sorting of large amount of data'', thereby ending the diagnostic process. Instead, \oursys cross-references with the query optimization knowledge, and then finds the correlated-subquery structure might be the performance bottleneck, with additional extracted information like estimated operation costs.
\end{sloppypar}

Third, {\it \llm+Metrics} meet trouble in deriving appropriate solutions. {\it \llm+Metrics} often gives very generic optimization solutions (e.g., ``resolve resource contention issues''), which are useless in practice. Instead, leveraging its \emph{tool retrieval} component, \oursys can learn to give specific optimization advice (e.g., invoking query transformation rules, adjusting the work\_mem parameter) or gather more insightful information (e.g., ``calculate the total cost of the plan and check whether the cost rate of the sort or hash operators exceeds the cost rate threshold'').


This evaluation reveals the potential of \oursys in going beyond mere anomaly detection to root cause analysis and provision of actionable suggestions. Despite these advancements, from the basic deployment of \oursys, there are still some unresolved challenges. First, it is tricky to share the maintenance experience (e.g., varying metric and view names) across different database products. Second, it is labor-intensive to adequately prepare extensive number of anomaly-diagnosis data, which is essential to fine-tune and direct less-capable \llms (e.g., those smaller than 10B) to understand the complex database knowledge and apply in maintenance.

%The unique ``tree of thought'' strategy of \oursys enables it to retrace previous steps and embark on a new line of investigation when faced with a failure. Furthermore, \oursys embodies an innovative approach to collaborative diagnosis, facilitating communication between multiple large language models to offer robust solutions through debate-like interactions. Consequently, \oursys not only delivers accurate diagnosis but also emphasizes system robustness and adaptability.


\iffalse
\begin{table}[]
	\small
	\caption{Diagnosis Results.}
	\label{tab:diag}
	%\vspace{-1em}
	\begin{tabular}{|c|l|l|l|}
		\hline
		Type                                                                              & \multicolumn{1}{c|}{Root Causes} & \textit{LLM+Metrics}      & \textit{D-Bot}            \\ \hline
		{DataInsert}                                                                        & INSERT\_LARGE\_DATA              &     $\times$                      & \checkmark \\ \hline
		\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Slow\\ Query\end{tabular}}             & FETCH\_LARGE\_DATA               &       $\times$                    & \checkmark \\ \cline{2-4} 
		& REDUNDANT\_INDEX    &   $\times$                        &          $\times$                 \\ \cline{2-4} 
		& LACK\_STATISTIC\_INFO            &    $\times$                       &            $\times$               \\ \cline{2-4} 
		& MISSING\_INDEXES                 & \checkmark & \checkmark \\ \cline{2-4} 
		& POOR\_JOIN\_PERFORMANCE          & \checkmark & \checkmark \\ \cline{2-4} 
		& STRING\_MATCHING                 &    $\times$                       & \checkmark \\ \cline{2-4} 
		& CORRELATED\_SUBQUERY             &    $\times$                       & \checkmark \\ \hline
		\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Concurrent\\ Transaction\end{tabular}} & LOCK\_CONTENTION                 &  $\times$                         &          $\times$                 \\ \cline{2-4} 
		& WORKLOAD\_CONTENTION             &    $\times$                       & \checkmark \\ \cline{2-4} 
		& CPU\_CONTENTION        & \checkmark & \checkmark \\ \cline{2-4} 
		& IO\_CONTENTION         & \checkmark & \checkmark \\ \hline
	\end{tabular}
	\vspace{-1em}
\end{table}

\begin{sloppypar}
Analyzing various root causes, \oursys outperformed the baseline across multiple categories. Specifically, within the \textit{``Data Insert''} root causes, it accurately diagnosed the \textit{'INSERT\_LARGE\_DATA'} issue, a feat the baseline system failed to achieve. Furthermore, under the \textit{``Slow Query''} category, \oursys identified not only the common root causes such as \textit{``MISSING\_INDEXES''} and \textit{``POOR\_JOIN\_PERFORMANCE''}, but also successfully diagnosed complex root causes like \textit{``FETCH\_LARGE\_DATA''} and \textit{``CORRELATED\_SUBQUERY''}, which the baseline overlooked. It should be noted that both \oursys and the baseline couldn't identify issues like \textit{``REDUNDANT\_INDEX''} and \textit{``LACK\_STATISTIC\_INFO''}. 
\end{sloppypar}

\begin{sloppypar}
Inspecting the \textit{``Concurrent Transaction''} category, \oursys demonstrated its superiority by correctly diagnosing \textit{``WORKLOAD\_CONTENTION''}, while the baseline fell short. However, both systems failed to identify \textit{``LOCK\_CONTENTION''}.
\end{sloppypar}


\fi


==> 06-methodology.tex <==
%!TEX root = ../main.tex
\section{Operators}
\label{sec:methodology}

\todo{Fix context: after optimization}

As shown in Fig.~\ref{fig:architecture}, the core function of each physical operator relies on an LLM core. \sys compile a configuration $c$ needs to an executable $e$. In the case of directly querying LLM, the configuration is compiled into an initial prompt for every input instance and the resulting executable is an interactive dialogue between the \sys system and the LLM. In the case of code generation, the configuration is compiled into a program (e.g., in Python) once and could be applied efficiently for loads of inputs.

\subsection{Direct Query}
\label{sec:direct-query}

Any procedure inside a data science application could always be viewed as a black-box function $f: X \to Y$. A straightforward approach to utilizing LLMs is to directly request $Y$ given $X$. This end-to-end method is effective for most cases, particularly when the task is simple but requires domain-specific knowledge.

For direct LLM queries, the configuration $c_{DQ} = (P,d_t,d_i,d_o,E,A,V)$ comprises a prompt template $P$, a natural language task description $d_t$, input and output type descriptions $d_i$ and $d_o$, an optional list of examples $E$, an optional set of adaptors $A$ (Sec.~\ref{sec:adaptor}), and an optional list of validators $V$. Given a new input $i$, the configuration parses $P$ using $d_t,d_i,d_o,E,A$, and $i$ to generate an initial prompt $p_i^0$ for the LLM. The final LLM response is validated by $V$ and then used as the output after one or multiple rounds of interaction.

The default standard prompt template $P$ involves a single interaction round, where the LLM directly provides the desired output. However, for more complex tasks, the LLM may require additional planning and reasoning. Chain-of-Thought Prompting (CoT)~\cite{cot} addresses this by explicitly guiding LLMs through intermediate thinking steps before reaching a conclusion. During this process, the LLM sequentially appends $p_i^1, p_i^2, \cdots$ to the initial prompt $p_i^0$ until a successful final confirmation $p_i^j$ is made.

Multi-round interactions can also enable the use of external tools. Naïve CoT prompting generates a static plan, which cannot leverage environmental knowledge. ReAct~\cite{react} addresses this by formulating multi-step reasoning with interaction as thoughts, actions, and observations. Actions execute plans, observations represent environmental feedback, and thoughts are internal actions that do not affect the environment. Reflexion~\cite{reflexion} extends ReAct by incorporating a reinforcement learning-based procedure, introducing a second LLM as an instructor that provides heuristics based on the actor LLM's actions and environmental rewards. The actor LLM can then use these heuristics to improve its planning and actions.

In \sys, the system interacts with the LLMs by providing adaptors (Sec.~\ref{sec:adaptor}) that serve as interfaces for LLMs to access local data and conventional data science tools, and validators (Sec.~\ref{sec:validator}) that provide feedback on the correctness of LLM responses. This design enables the further extension of the Reflexion pipeline, with adaptors supplying observations and validators offering environmental rewards and heuristics.

\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/direct_query.pdf}
  \caption{Direct Query: An NL2SQL Example.}
  \Description{...}
  \label{fig:direct-query}
\end{figure}

\sys supports three types of prompt templates: standard prompt, CoT prompt, and fully-interactive prompt. The standard prompt is sufficient for simple tasks and is used as the default when no adaptors are provided. For complex tasks, a CoT prompt can be employed to enhance effectiveness. However, in most cases, when adaptors are available, \sys utilizes the fully-interactive prompt to coordinate between the LLM and local data. Specifically, the initial prompt $p_i^0$ is generated with additional information provided: the set of available adaptors $A$. During each interaction round $j$, given $p_i^0,p_i^1,\cdots,p_i^{j-1}$, the LLM first generates thought $t_i^j$ and action $a_i^j$. The action either involves invoking an adaptor from $A$ or confirming the final response. An observation $o_i^j$ is returned, which could be the local data or function supplied by the invoked adaptor. Consequently, $(t_i^j,a_i^j,o_i^j)$ together form the next prompt $p_i^j$. Finally, the list of validators $V$ would provide feedback $S$ in case of an incorrect final response to refine the initial prompt $p_i^0$. (Fig.~\ref{fig:direct-query})

\subsection{Code Generation}
\label{sec:code-generation}

In addition to directly querying LLMs for accessing their common sense knowledge, another way to leverage LLMs is through code generation. This approach enables the swift and adaptive development of new data science applications. While direct querying of LLMs can be effective, it may not be feasible to process every data record using LLMs in certain sub-processes of a data science application that involve a massive amount of local data. Compared to directly querying LLMs, employing LLM-generated code locally can be more efficient. Compared to manually written code, LLM-generated code offers enhanced flexibility, as it can adapt to changing requirements and data formats.

However, most mainstream LLMs are not yet suitable for producing complex logic or building large-scale applications, as they are only capable of generating small pieces of code. To address this scalability issue, \sys emphasizes modularization and tool utilization to connect separate code pieces.

\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/code_generation.pdf}
  \caption{Code Generation: A Name Extraction Example.}
  \Description{...}
  \label{fig:code-generation}
\end{figure}

For code generation, the configuration $c_{CG} = (P,d_t,d_i,d_o,E,A,V)$ is compiled into a local program function $r(\cdot)$, which can be independently applied to a list of inputs to obtain the corresponding outputs $o = r(i)$. Similar to directly querying LLMs, the configuration parses $P$ into the initial prompt $p_i^0$. The key difference is that the code of program $r$ is returned by the LLM with all the adaptors already considered. The subsequent interactions come from the validators $V$, whose feedback as well as the current program $r$ together compose the prompts $p_i^j$ to revise the generated code. (Fig.~\ref{fig:code-generation})

The significance of tool utilization in LLM-generated code cannot be overstated. As a crucial area of research, tool utilization has been gaining attention alongside recent advancements in LLMs. Previous studies~\cite{visual-chatgpt,hugginggpt} have primarily concentrated on prompt engineering to tackle the planning and decision-making aspects of tool utilization. However, in our context, high-level logical operators and user instructions predominantly dictate the planning process. Consequently, a more pressing concern is to accurately define and describe the tools.

In our \sys, tools encompass: open-ended tools, which refer to publicly available resources that LLMs can access, such as common Python packages; user-provided tools, which include APIs for local data science functions; and custom operators. LLMs inherently support open-ended tools through their pretraining process, while in \sys, user-provided tools and custom operators are managed via adaptors.

It is important to note that the code generation process in \sys not only produces a single piece of code in textual format but also records additional information to facilitate advanced modifications to the code. In technical terms, a generated executable comprises a list or tree of versions, where each version includes the code, linked to a specific programming language (such as Python), and the corresponding prompt used for generating that version. The preservation of historical code and prompts not only allows for efficient version control but also enables the integration of validators (Sec.~\ref{sec:validator}) and ensemblers (Sec.~\ref{sec:ensembler}) to improve the overall performance.

==> 07-future.tex <==
%!TEX root = ../main.tex


%todo
\section{Other Opportunities}
\label{sec:opportunities}


==> 07-insights.tex <==
%!TEX root = ../main.tex

\section{Summarization}
\label{sec:summary}

From above case study, we can see $(i)$ \oursys can well cover diversified applications (especially in data management area) and $(ii)$ different applications can customize the adopted components in \oursys to fit their scenario characters. For example

(1) Applications like data cleaning require a vast number of different data sources, which involve many subtasks and may process various user requests. Instead, query rewrite application mainly relies on rewrite rules and its request parsing module is also much simpler. However, the scheduling of execution plan of query rewrite is much more tricky than applications like data cleaning.



==> 07-processing.tex <==
%!TEX root = ../main.tex
\section{Data Processing}
\label{sec:processing}

In the rapidly expanding field of data science, researchers often find themselves dedicating a substantial portion of their time and effort to preprocessing the heterogeneous data they encounter. The preprocessing stage, therefore, serves as a crucial step in transforming raw data into a clean, well-structured format for further analysis. With the help of LLMs, \sys has developed multiple methods in improving the processing and understanding of user-specified local data.

\subsection{Automatic Preprocessing}
\label{sec:pre-processing}

First of all, when assuming that the local data, or a part of the local data is homogeneous and in serializable format, \sys could directly use the code generation operator to specify a \texttt{LOAD\_DATA} operator.

\subsubsection{Processing of Long Textual Data}
\label{sec:long-text}

\subsubsection{Processing of Knowledge Graphs}
\label{sec:knowledge-graphs}

\subsubsection{Data as Local Search Engine}
\label{sec:search-engine}

\subsubsection{Data as Structured Database}
\label{sec:sql}

\todo{}

\subsection{Generation}
\label{sec:generation}

\todo{}

\subsection{Annotation}
\label{sec:annotation}

\todo{}


==> 08-implementation.tex <==
%!TEX root = ../main.tex
\section{Implementation Details}
\label{sec:implementation}

\todo{Implementation Details: Python sandbox, prompt details, etc.}

==> 08-relatedwork.tex <==
%!TEX root = ../main.tex

\section{Related Work} \label{sec:relatedwork}


Recently, there are attempts in applying large language models (\llms) in data management tasks: $(i)$ For data augmentation, there are works that utilize zero/few-shot techniques to remove duplicate tuples and impulse missing values in origin datasets~\cite{DBLP:journals/pvldb/NarayanCOR22,DBLP:conf/icde/ZhangFCKMBPP23,li2023table,DBLP:journals/corr/abs-2312-03987}; $(ii)$ For query rewrite, there are works that test the rewriting capability of \llm by generating basic task descriptions~\cite{DBLP:journals/corr/abs-2305-03111} or heuristically polishing the descriptions for better performance~\cite{zhoudb}; $(iii)$ For data analytics, there are works that utilize tools like Pandas to generate basic analysis code~\cite{qin2023tool,DBLP:journals/corr/abs-2306-01499}.  

These works shield light on opportunities of {\it LLM4DB}. However, as declared by openai ``ChatGPT can make mistakes. Consider checking important information'', which is not sufficient for building a prototype of industry system. 


==> 09-experiments.tex <==
%!TEX root = ../main.tex
\section{Experiments}
\label{sec:exp}

\todo{quantitative experiments: accuracy, efficiency, \#llm calls}

\todo{ablation on the core components}

\todo{multiple tasks: topic classification, imputation, entity resolution, NL2SQL, fancy example (map?), extraction (evaporate?), database operation}

==> 10-conclusion.tex <==
%!TEX root = ../main.tex
\section{Conclusion}
\label{sec:conclusion}

\todo{Conclusion}

\todo{Limitation}

==> challenges.tex <==
%!TEX root = ../main.tex

\section{Research Challenges}
\label{sec:challenges}

\noindent {\it (C1) Maximizing Data Utilization.} Assuming we have some well prepared data sources (e.g., historical data cleaning examples), it is vital make the system understands and fully utilizes the data, i.e., $(i)$ when to utilize the data (e.g., application scenarios), $(ii)$ how to utilize the data (e.g., SQL language for relational data), and $(iii)$ how to transform the data formats to ease  understanding of the proxy model (\llm) in prompt and training level.

\noindent {\it (C2) Clarifying Ambiguous Requests.} Different from SQL statements or Spark jobs, natural language requests generally do not content clear requirements and target data sources. Thus, from the raw request, it is vital to derive entities like $(i)$ the target data or model sources, $(ii)$ lookup constraints, and $(iii)$ output results.

\noindent {\it (C3) Managing Execution Operations.} First, how to encapsulate atomic operations that are commonly utilized for the specific task, which are vital to split a complex task request into operation chains that greatly improve the system stability. Second, similar to Spark Jobs, how to organize task operations in a computation graph structure that can greatly increase the task-solving efficiency.

==> data-clean.tex <==
%!TEX root = ../main.tex

\begin{figure}[!t]
	\vspace{-.5em}
	\centering
	\includegraphics[width=.95\linewidth, trim={0 0 0 0},clip]{./figures/case-data-clean.pdf}
	\vspace{-.5em}
	%\captionsetup{skip=0pt}
	\caption{\oursys for Data Cleaning}
	\label{fig:data-clean}
	\vspace{-1.5em}
\end{figure}

\section{\oursys for Data Cleaning}
\label{sec:data-clean}

Data cleaning involves tasks like correcting inaccurate data, removing duplicate data, modifying incorrectly formatted data. And it is a typical application that heavily relies on human analysts for critical steps, such as aligning semantically-similar attributes (e.g., understanding that acronyms like ``first name'' and ``name'' both refer to a person's first name and can be combined)~\cite{DBLP:conf/icde/ChaiF0WZ19,tang2020rpt}, which are possible to handle by \llm workers. As shown in Figure~\ref{fig:data-clean}, we showcase how to conduct data cleaning using \oursys.

\hi{Preparation.} First, we collect from multiple sources, including $(i)$ a vast number of matching entities and non-matching entities (in relational database), $(ii)$ a set of data cleaning questions (in vector database), $(iii)$ data cleaning experience from open websites and human analysts (in vector database), and $(iv)$ relevant training datasets and models like~\cite{tang2020rpt}. Next, we extract keywords that frequently occur within these sources, such as synonyms for the entity matching task. Finally, we initialize the keyword-API mapping table based on the available cleaning APIs (e.g., Dedupe.io API for duplicate entity resolving~\cite{dedupe}).

%\textit{(1) Format Standardization:} Ensuring consistent data formats across a dataset. For example, standardizing dates to a single format (e.g., converting "DD-MM-YYYY" and "MM/DD/YYYY" to a uniform format) is essential for accurate data analysis and comparison.

%\textit{Example 2:} Different representations of phone numbers, some with country codes and others without.

%\textit{(1) Outlier Detection} involves entities that significantly deviate from the majority. For example, in a dataset of temperatures, an entity of -5°C is an outlier when most values are between 20-30°C. %Such outliers can indicate data entry errors or unique, significant events worth investigating.

%\textit{Example 2:} In a dataset of employee ages, where most entries are between 25 and 60 years, an entry is listed as 120 years.

%\textit{(2) Missing Value Imputation:} This process deals with filling in missing or incomplete data. For example, a sales report missing the `Date of Purchase' field for some entities. %Efficient imputation helps in maintaining the integrity and usability of the dataset.

%\textit{Example 1:} A customer database with missing email addresses in some records.

%\textit{(3) Duplicate Detection:} This task involves identifying and resolving duplicate entities. For example, two entities in a contact list with slightly different names (e.g., "Jon Doe" and "John Doe") but identical phone numbers. %This is crucial for maintaining a clean, non-redundant dataset.


\hi{Request Pre-Processing.} Giving a data cleaning request ({\it ``Are $E_1$ and $E_2$ the same? Why?''}), we pre-process the request into a format that is easy to deduce into operations, i.e., $(i)$ We detect ``Compare'' and map it to the ``entity matching'' operation; $(ii)$ We locate source-relevant keywords like ``[title], [id]'' attributes and enrich with the source information like {\it ``[title], [id] features from [dataset A]''}; $(ii)$ Add additional knowledge for above terms, such as the criteria for the matching operations and even the predicates for filtering entities accessed from the datasets. Besides, if it decides some information (e.g., {\it ``within [location] under [price range]''}) is missing, it can further ask the user to provide.

\hi{Request Parsing.} Next, with the enriched question, we map the terms or sentences within the question into operations according to items like ``retrieve'' and ``compare''. For each operation, we add metadata information like the source name and whether reusing cached results. In this way, we derive three operations to execute.

\hi{Request Execution.} With the derived operations, we organize them as an execution plan to carry out from bottom up. That is, we first access $(i)$ relational database to obtain entity pairs with similar schema and $(ii)$ knowledge from the vector database. For each access operation, we append an \llm proxy to judge whether the input entities are similar and give reasons according to the relevant entities or knowledge. Afterward, we bring in the merge operation to decide the finial answer, where the \llm can also refer to previous data cleaning cases.

%  according to outputs from the two proxy models

\hi{Data and Model Management.} For the given question, if there are no similar questions in existing sources, we can persist them in both relational database (entities) and vector database (textual question) and fine-tune models with newly incoming entities and questions in batch.

\hi{Research Challenges.} 


\iffalse
\subsection{LLM for Data Cleaning}

In the context of data cleaning, LLMs are trained to tackle tasks such as outlier detection, missing value imputation, and duplicate detection. To create a robust training dataset, it is crucial to generate samples that trigger real-world data cleaning operations:

%accurately reflect real-world data inconsistencies. This dataset should cover a range of irregularities, including but not limited to outliers, incomplete entries, and format inconsistencies:


%\textit{Example 2:} Repeated rows in a transaction log due to a system error.

The initial samples can be generated via $(i)$ collecting from existing datasets (e.g., in GitHub) and $(ii)$ prompting \llms to synthesize samples based on the large pre-training corpus.

\noindent \bfit{Collection from Existing Datasets:} This involves using datasets from repositories like GitHub, Kaggle, or proprietary databases. These datasets, often containing real-world inconsistencies, serve as a rich source for understanding the typical errors and irregularities that need addressing. For instance, the Enron Email Dataset is an extensive collection of over 600,000 emails from the employees of the Enron Corporation. Data cleaning tasks in this dataset involve filtering, categorizing, and extracting meaningful information from a vast collection of unstructured email data.

%\textit{Example 2:} Analyzing datasets from Kaggle competitions, which often include real-world data with common inconsistencies.

\noindent \bfit{Synthesis using \llms:} \llms, trained on vast corpora of data, can generate synthetic data samples that mimic real-world inconsistencies. This approach is particularly useful for creating samples that are hard to find in existing datasets or for simulating rare but critical data irregularities. For instance, an \llm can be programmed to introduce errors such as transposing letters in names or misaligning fields in a structured dataset. 

%A specific scenario could involve an LLM generating a dataset of customer records where the 'FirstName' and 'LastName' fields are occasionally swapped, or numerical values like zip codes are inconsistently formatted. This artificially created data then serves as a testing ground for developing and refining data cleaning algorithms capable of correcting such errors.


%\textit{Example 2:} Creating synthetic datasets with intentionally misplaced or missing values to train models on handling such scenarios.


%This approach helps in fine-tuning the model's accuracy on more complex or nuanced data points. On the other hand, 

%The training is augmented through active learning, where the model is iteratively refined based on its performance in identifying and rectifying data anomalies.

\subsection{Reasoning Chains for Data Cleaning}

Within the reasoning chain, the agent utilizes finetuned \llm to decide a series of data cleaning components (e.g., standardization rules, entity matching actions). These chains are designed to tackle different aspects of data cleaning in a coordinated manner. For example, one chain might focus on normalizing data formats, while another could specialize in identifying and merging duplicates.

% For the agent, it needs to assess, prioritize and execute cleaning processes based on the specific needs of the dataset, and dynamically adjusts the sequence of operations to maximize cleaning efficiency and accuracy.

Consider a scenario where the dataset containing customer information from various sources. The first step is to assess the dataset to identify inconsistencies and errors. The agent detects variations in date formats (DD/MM/YYYY in some entries, MM/DD/YYYY in others) and decides to normalize all dates to the ISO format (YYYY-MM-DD). Next, it identifies duplicate records based on name and address fields. The agent prioritizes merging these duplicates, ensuring no data loss by comparing and consolidating field values. After addressing duplicates, the agent examines the email addresses, applying a regex pattern (under the guidance of humans probably) to validate their format and flagging any invalid entries for review. In the final step, the agent reassesses the dataset, ensuring all changes have improved its overall quality and consistency."


\subsection{VDB for Data Cleaning}

In data cleaning, the Vector Database (VDB) operates as a dynamic cache mechanism. It stores  embeddings which represent various descriptions of data cleaning tasks and their corresponding processing strategies. This setup accelerates the selection of appropriate data cleaning tools (e.g., {\it OpenRefine} for data transformation and {\it Trifacta} for pattern discovery). For instance, suppose the VDB contains embeddings for tasks such as duplicate detection ({\it DuplicateFinder}), format normalization ({\it FormatNormalizer}), and outlier identification ({\it OutlierDetector}). When a new data cleaning task is introduced, the system generates an embedding for this task and compares it with the existing embeddings in the VDB using similarity measures (e.g., BM25~\cite{robertson2009probabilistic}). The top-K tools whose task embeddings are most similar to the new task's embedding are selected to integrate into the \llm's prompt.

Moreover, VDB serves as a repository of domain knowledge, augmenting data cleaning processes with contextual understanding. For instance, VDB might use historical data patterns to guide the imputation of missing values, ensuring that the imputed data aligns with domain-specific trends and norms. Specifically, consider a dataset in the healthcare domain with missing blood pressure readings. VDB, utilizing its repository of patient histories and typical blood pressure ranges, can intelligently impute these values based on age, weight, and other related health indicators.



\section{\lvc For Data Cleaning}
\label{sec:data-clean}

\subsection{\llm for Data Cleaning}

Data cleaning tasks include outlier detection and imputation, missing value imputation, duplicate detection. We need to teach LLM for understanding data cleaning tasks. To this end, we need to generate some training examples. The challenge here is how to generate representative examples. We use active learning techniques.

\subsection{Chains for Data Cleaning}

Components are data cleaning tools.
Each chain is a sequence of calling tools.
Agent is ToT of scheduling. How to train the ToT.


\subsection{\vdb for Data Cleaning}

We act VDB as a caching, which cache the embedding of a cleaning task and the corresponding value is the next DSL that to be used.
VDB can also be acted as a domain knowledge augmentation. 

\fi
